Navigating the Future of Federated Recommendation Systems with Foundation Models

Federated Recommendation Systems (FRSs) offer a privacy-preserving alternative to traditional centralized approaches by decentralizing data storage. However, they face persistent challenges such as data sparsity and heterogeneity, largely due to isolated client environments. Recent advances in Foundation Models (FMs), particularly large language models like ChatGPT, present an opportunity to surmount these issues through powerful, cross-task knowledge transfer. In this position paper, we systematically examine the convergence of FRSs and FMs, illustrating how FM-enhanced frameworks can substantially improve client-side personalization, communication efficiency, and server-side aggregation. We also delve into pivotal challenges introduced by this integration, including privacy-security trade-offs, non-IID data, and resource constraints in federated setups, and propose prospective research directions in areas such as multimodal recommendation, real-time FM adaptation, and explainable federated reasoning. By unifying FRSs with FMs, our position paper provides a forward-looking roadmap for advancing privacy-preserving, high-performance recommendation systems that fully leverage large-scale pre-trained knowledge to enhance local performance.

==> TKDE/sections/sec_app.tex <==
%!TEX root = ../main.tex

\section{Applications}
\label{sec:app}

\subsection{eHealthcare Systems}
 eHealthcare systems leverage modern technology to enhance the quality and efficiency of medical services, such as remote diagnosis and patient monitoring. Federated recommendation systems allow different medical institutions to share insights from patient data without sharing the data itself, which is crucial for protecting sensitive health information. Generative models use this data to provide doctors and patients with personalized treatment plans and health advice, improving diagnostic accuracy and treatment outcomes. Thus, federated recommendation systems combined with generative models can integrate patient health data across institutions to create complex treatment pathways and simulate disease progression, enabling doctors to better predict patients' responses to specific treatments and provide more precise medical services.

\subsection{Industrial Applications}
In manufacturing, automation and intelligent technologies significantly enhance production efficiency and safety. Federated recommendation systems foster technological collaboration between different enterprises by sharing non-sensitive data, accelerating product design and optimization processes. This not only shortens product development cycles but also protects corporate trade secrets. Generative models can design new mechanical parts or product prototypes by simulating different design variables, quickly proposing multiple design solutions; they can also help predict machine failures, perform maintenance in advance, and reduce downtime, thereby enhancing production efficiency. Federated recommendation systems combined with generative models enable the sharing of improvements and innovations while maintaining data privacy between companies.

\subsection{Consumer Services}
Analyzing consumer behavior helps businesses deeply understand customer needs. Federated recommendation systems can integrate data from different service providers while protecting user privacy, achieving personalized services. Generative models provide personalized recommendations based on this data, enhancing user experience. For example, in travel recommendation systems, models generate customized travel itineraries based on users' historical preferences. By simulating different consumer behavior patterns, businesses can predict market trends, adjust service strategies, and enhance competitiveness. Federated recommendation systems combined with generative models analyze user behavior data from different service providers to generate service plans that meet individual needs, promoting personalized service development.

\subsection{Retail and E-commerce}
Applying recommendation systems to online shopping and retail provides a personalized shopping experience. Federated recommendation systems in the retail and e-commerce sectors analyze consumer shopping habits to generate personalized product recommendations, increasing users' purchasing desire and satisfaction. Retailers and e-commerce platforms can use generative models to predict consumer buying behavior, thereby offering more accurate product recommendations, optimizing inventory, and enhancing sales efficiency. Federated recommendation systems combined with generative models allow retailers and e-commerce platforms to consider market conditions comprehensively, predicting consumer buying behavior and providing more precise product recommendations, optimizing inventory, and enhancing sales efficiency.

\subsection{Finance and Banking}
In the financial sector, recommendation systems use data analysis and prediction models to optimize financial services, applicable for credit assessments, stock market analysis, etc., offering clients tailored financial products. Federated recommendation systems ensure transaction data privacy while offering clients tailored financial products. Generative models can simulate market behaviors, predicting stock prices or financial product returns. These models help financial institutions formulate more accurate investment strategies while reducing risks. In finance, federated recommendation systems combined with generative models help financial institutions protect client privacy while simulating market changes and user behavior, offering advice on investment products and credit strategies, thereby enhancing clients' investment returns and satisfaction.

\subsection{Smart Cities}
In smart city applications, systems need to process and analyze large-scale urban data. From optimizing traffic flow to devising public safety strategies, federated recommendation systems can help city planners use resident data without directly sharing it to recommend strategies for improving public services and infrastructure, enhancing urban management efficiency and improving residents' quality of life. Additionally, using generative models to simulate the effects of different strategies can find optimal solutions for managing and allocating urban resources. For example, by simulating traffic flow, models can predict congestion and propose solutions, improving urban traffic efficiency. Federated recommendation systems combined with generative models can help city planners optimize resource allocation and management efficiency without sharing resident data.

\subsection{Social Networking}
 Social platforms facilitate interpersonal communication and information sharing online, using recommendation systems to suggest content to users, such as friends or topics of interest, to increase user engagement. Federated recommendation systems can enhance user engagement and satisfaction while protecting user privacy. Generative models can generate personalized content recommendations, enhancing user engagement and satisfaction while ensuring the protection of user privacy, increasing platform attractiveness and user retention.

\subsection{Education}
 In the field of education, using recommendation systems can improve teaching methods by making appropriate recommendations based on students' progress and abilities, providing a personalized learning experience. Generative models can generate personalized learning materials and courses based on students' progress and interests. These customized learning resources can enhance students' learning efficiency and interest. Federated recommendation systems combined with generative models can generate personalized learning paths based on students' feedback and learning history. By simulating teaching scenarios and student learning processes, these systems can provide resources that better meet individual learning needs.



==> TKDE/sections/sec_bg.tex <==
%!TEX root = ../main.tex

\begin{figure*}[!t]
    \centering
    \includegraphics[width=.9\textwidth]{figures/tax_frs_fm.pdf}
    \caption{
        The taxonomy of FRS and FM frameworks categorized by their respective core criteria in Sec. \ref{sec:bg}.
    }
    \label{fig:tax}
\end{figure*}


\section{Background and Preliminary}
\label{sec:bg}

To provide a comprehensive understanding of the integration of FRSs and FMs, this section outlines their core principles, taxonomies, and foundational structures, as illustrated in Fig. \ref{fig:tax}, establishing a basis for analyzing their synergies.


\subsection{Federated Recommendation System}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/typical_FRS.png}
    \caption{
        A framework for FRSs, illustrating client-side local training with private data, server-side global aggregation, and update communication. 
        Local models integrate user and item embeddings with prediction networks, while the server aggregates the sent local updates to enhance the global model, ensuring privacy and personalization.
        }
    \label{fig:typical_FRS}
\end{figure}

\begin{definition}[Federated Recommendation System]
\label{def:frs}
A Federated Recommendation System is a technology that uses distributed algorithms for personalized information filtering. It aims to improve the accuracy of information filtering and the effectiveness of personalized services, while maintaining user privacy.
\end{definition}

FRSs enable collaborative learning across multiple clients without direct exchange of raw user data. 
Fig. \ref{fig:typical_FRS} illustrates that FRS typically involves three key processes: 1) client model update, 2) communication, and 3) global aggregation. 
Users train models locally using their own data and share updated parameters (e.g., gradients) with a server. 
The server then performs global aggregation, integrating information from all participants and redistributing updated parameters. 
This communication process preserves privacy and security.

\begin{figure*}[!t]
    \centering
    \subfloat[Horizontal FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_horizontal.png}
        \label{fig:horizontal_frs}
    }\hspace{10pt}
    \subfloat[Vertical FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_vertical.png}
        \label{fig:vertical_frs}
    }\hspace{10pt}
    \subfloat[Transfer FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_transfer.png}
        \label{fig:transfer_frs}
    }
    \caption{
        Typical data distribution paradigms in FRS: 
        (a) Horizontal FRS, characterized by similar feature spaces across users but distinct data samples; 
        (b) Vertical FRS, involving overlapping user sets with disparate feature spaces; 
        and (c) Transfer FRS, leveraging transfer learning to enable knowledge sharing across domains with limited or complementary data distributions.
    }
    \label{fig:data_type}
\end{figure*}

As illustrated in Fig. \ref{fig:tax}, FRSs can be categorized based on data distribution and communication architecture \cite{yang2020federated,sun2024survey}.

\subsubsection{Data Distribution Paradigms in FRS}
There are three categories based the data distribution, each addresses specific data collaboration and learning scenarios:
\begin{itemize}
    \item \textbf{Horizontal FRS} deals with similar feature spaces but different sample spaces, as shown in Fig. \ref{fig:horizontal_frs}. 
    It aggregates model updates from multiple clients to train recommendation models while preserving privacy~\cite{zhang2023dual,li2024federated,zhang2024federated}.
    
    \item \textbf{Vertical FRS} 
    is applied when feature spaces differ but sample spaces are similar, as shown in Fig. \ref{fig:vertical_frs}. 
    It securely integrates different data types (e.g., a bank's credit history) to enrich user information \cite{zhang2021vertical,cao2023privacy,mai2023vertical,wan2023fedpdd}.
    
    \item \textbf{Transfer FRS} 
    utilizes transfer learning \cite{zhuang2020comprehensive} to transfer knowledge from one domain to another, benefiting scenarios with limited data for independent model training \cite{zhang2024transfr}, shown in Fig. \ref{fig:transfer_frs}.

\end{itemize}

Each type of FRS based on data distribution is designed to address specific collaboration scenarios, ensuring privacy and efficient learning. 
Horizontal FRS is suitable for situations where similar features are available across clients, Vertical FRS integrates different types of features for the same users, and Transfer FRS allows knowledge transfer across domains, making it particularly useful when data is scarce.

\begin{figure*}[!t]
    \centering
    \subfloat[Centralized FRS]{
        \label{fig:arch_cent}
        \includegraphics[width=.6\columnwidth]{figures/type_traditional.png}
    }\hspace{5pt}
    \subfloat[Semi-decentralized FRS]{
        \label{fig:arch_semi}
        \includegraphics[width=.6\columnwidth]{figures/type_semi-decentralized.png}
    }\hspace{5pt}
    \subfloat[Decentralized FRS]{
        \label{fig:arch_decent}
        \includegraphics[width=.6\columnwidth]{figures/type_decentralized.png}
    }
    \caption{
        Architectural paradigms of FRS: 
        (a) Centralized FRS, relying on a central server for model aggregation; 
        (b) Semi-decentralized FRS, incorporating intermediate nodes to balance scalability and efficiency; 
        and (c) Decentralized FRS, enabling peer-to-peer communication to enhance privacy and robustness.
    }
    \label{fig:archi_type}
\end{figure*}

\subsubsection{Communication Architectures in FRS}
As shown in Fig. \ref{fig:archi_type}, 
Based on communication architecture, FRS can be categorized into centralized, semi-decentralized and decentralized based on their communication architecture. Each type addresses privacy and scalability in different ways:
\begin{itemize}
    \item \textbf{Centralized FRS}: 
    A central server orchestrates the learning process in Fig. \ref{fig:arch_cent}, simplifying model aggregation to overcome data silo issues~\cite{li2022federated} while relying on a central authority. 
    This approach is straightforward but depends heavily on the central server, creating a single point of failure and potential privacy risks \cite{zhang2023lightfr,zhang2023dual,li2024federated,zhang2024federated,zhang2024transfr}.
    
    \item \textbf{Semi-decentralized FRS}: 
    As shown in Fig. \ref{fig:arch_semi},
    It introduces an intermediate layer (e.g., edge servers) to reduce communication overhead and enhance scalability. 
    This architecture balances the advantages of centralized and decentralized systems, improving system efficiency while still managing privacy concerns~\cite{qu2023semi}.
    
    \item \textbf{Decentralized FRS}:
    It employs peer-to-peer communication~\cite{hegedHus2019decentralized}, which maximizes privacy but necessitates complex coordination. 
    As illustrated in Fig. \ref{fig:arch_decent}, each client communicates directly with others without relying on a central server. This enhances privacy and reduces dependence on a single entity; however, it comes at the expense of increased communication complexity and the requirement for robust consensus mechanisms \cite{zheng2023decentralized,li2024decentralized}.

\end{itemize}

Each of these architectures offers a trade-off between privacy, communication efficiency and the degree of decentralization. 
Centralized systems simplify model aggregation, but rely on a central authority. 
Semi-decentralized systems aim to balance efficiency and privacy with an intermediate layer, while decentralized systems offer the highest level of privacy at the cost of more complex model coordination.


\subsection{Foundation Model}

The rapid increase in the performance of computer hardwares, e.g., GPUs, the increasing maturity of transformer architectures, and the public availability of large amounts of training data have been three key factors in the emergence of FMs~\cite{bommasani2021opportunities}. 
According to the work of Stanford HAI~\cite{bommasani2021opportunities}, we have the following definition of FMs:
\begin{definition}[Foundation Model]
\label{def:fm}
    A foundation model is defined as any model trained on extensive data (typically using large-scale self-supervised learning) that is capable of adapting to a wide range of downstream tasks, for instance, through fine-tuning or prompting.
\end{definition}

FMs are pre-trained on extensive data, enabling adaptation to a wide range of downstream tasks through fine-tuning or prompting \cite{church2021emerging,yuan2023power}.
These models, e.g. GPT-3 \cite{brown2020language}, are distinguished by two key characteristics \cite{bommasani2021opportunities}: 
1) \textit{Emergence}, refers to the model's ability to develop new capabilities from training data without explicit programming; 
and 2) \textit{Homogenization}, highlights the unified approach across diverse machine learning tasks, making FMs adaptable across multiple domains. 

Although FMs are based on self-supervised learning and transfer learning, their scale brings new emergent abilities, and their effectiveness in many tasks has motivated homogenization, e.g., many FMs have evolved based on transformer architectures \cite{devlin2018bert,liu2019roberta,dosovitskiy2020image,brown2020language}.
While homogenization provides strong leverage, it also requires caution, as defects in foundation models can be inherited by all downstream adapted models. 
Despite the broad deployment prospects of foundation models, due to their emergent properties, our understanding of how they work, when they fail, and what they can actually do is still quite limited \cite{bommasani2021opportunities}, but there has been quite a bit of work \cite{wei2022chain,yang2024foundation,zhao2024explainability} that attempts to explain this phenomenon.
Moreover, OpenAI proposes a Scaling Law for LLM \cite{kaplan2020scaling}, suggesting that the performance of a model is governed by a power-law relationship involving computational power, model parameters, and data size. This law also applies to downstream tasks \cite{isik2024scaling}. 
Therefore, understanding and leveraging this power-law relationship when using FM can aid in more efficiently allocating resources and optimizing model performance.

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=.8\columnwidth]{figures/tax_fm.png}
%     \caption{The diagram illustrates the taxonomy of FM based on two main criteria: Data Type and Functionality.}
%     \label{fig:tax_fm}
% \end{figure}

\subsubsection{Taxonomy of FM}
As shown in Fig. \ref{fig:tax}, similar to FRS, FMs can also be classified based on data type or functionality. 
Specifically, based on the type of data used during training, FM is mainly divided into followings \cite{bommasani2021opportunities}:
\begin{itemize}
    \item \textbf{Language FM}: 
    Trained on textual data to understand and generate language \cite{devlin2018bert,liu2019roberta}, excelling in natural language processing tasks such as machine translation \cite{dabre2020survey}, search \cite{lu2020twinbert,liu2021pre}, and sentiment analysis \cite{mathew2020review}.
    Typical language models include BERT \cite{devlin2018bert}, GPT-3 \cite{brown2020language}, and LLama \cite{touvron2023llama}, which typically use deep transformer architectures that are able to capture complex linguistic regularities and demonstrate excellent performance on multilingual tasks.
    
    \item \textbf{Vision FM}: 
    Focused on understanding image data, these models, such as DINOv2 \cite{oquab2023dinov2} and SAM \cite{kirillov2023segment}, are used for object recognition \cite{dosovitskiy2020image,wang2023all,zhang2023recognize}, visual reasoning \cite{huang2022perceive,ding2023visual} and image segmentation \cite{kirillov2023segment,wang2023seggpt,zou2024segment}.
    
    \item \textbf{Multi-modal FM}: 
    These models, e.g. CLIP \cite{radford2021learning} and DALL·E \cite{tamkin2021understanding}, integrate multiple types of data, such as text and images, allowing them to handle cross-modal tasks like image captioning and visual quizzing \cite{bai2023qwen,wang2023cogvlm,you2023ferret} by integrating information from different modalities. 
\end{itemize}

Functionally, FMs can be categorized into \cite{bommasani2021opportunities,liu2023towards,wu2023survey}:
\begin{itemize}
    \item \textbf{Discriminative FM}: 
    Primarily used for tasks like classification \cite{yao2022prompt,chen2023robust} and regression \cite{ali2023evaluating}, focusing on distinguishing between different classes of input data.
    
    \item \textbf{Generative FM}: 
    Such as GPT-3 and DALL·E, are designed to generate new data instances by learning the distribution of the training data \cite{cao2023comprehensive}, supporting applications like text \cite{otter2020survey} and image generation \cite{ho2022cascaded,saharia2022palette}.
\end{itemize}

Each type of FM offers unique advantages in its respective area. Language, vision, and multi-modal models provide specialized capabilities for processing different data types, while discriminative and generative models offer distinct approaches for solving problems based on either classification or data generation. By leveraging these specialized models, FMs can address a wide range of challenges across diverse domains.

\subsubsection{Adaptation}

Fig.~\ref{fig:fm} illustrates a commonly used technique for pre-trained models, known as the Adaptation. 
Adaptation is a commonly used technique for pre-trained models, where new lightweight layers are added while maintaining the original parameters of the pre-trained model. This enables fine-tuning and extension for specific tasks \cite{ding2023parameter,zhang2024federated}, making it suitable for multi-task learning and tasks performed in resource-limited environments, such as few-shot learning \cite{liu2024few}. 
Adaptation techniques have found wide applications in natural language processing and computer vision tasks \cite{hu2021lora,dettmers2024qlora,gao2024clip}.

Adaptations can be categorized into three main types \cite{liu2024few}:
\begin{itemize}
    \item \textbf{Prompt-based Fine-tuning Adaptation Methods}:
    These methods~\cite{zhou2022learning,zhou2022conditional} use prompt learning to adapt models for specific tasks by fine-tuning a portion of the fixed text input as a learnable vector. This allows the model to adjust quickly for new tasks with minimal changes.

    \item \textbf{Adapter-based Fine-tuning Adaptation Methods}: 
    Small, trainable modules, called Adapters, are added to a pre-trained model. 
    These adapters \cite{guo2023calip,gao2024clip,hu2021lora} are fine-tuned instead of the entire model, making task adaptation efficient with minimal parameter updates.

    \item \textbf{External Knowledge-based Adaptation Methods}:
    External knowledge, such as information from knowledge graphs or additional model queries, is integrated to improve the model's performance on domain-specific tasks, especially when data is limited \cite{pratt2023does,yang2023language}.

\end{itemize}

In summary, adaptations play a crucial role in enhancing the versatility of foundation models. By enabling efficient fine-tuning and leveraging external knowledge, these methods help foundation models effectively tackle a wide range of tasks, even in resource-constrained settings or when training data is scarce. This adaptability is key to making foundation models more practical and powerful for real-world applications.

==> TKDE/sections/sec_bg_old.tex <==
%!TEX root = ../main.tex

\section{Background and Preliminary}
\label{sec:bg}

\subsection{Federated Recommendation System}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.85\columnwidth]{figures/typical_FRS.png}
    \caption{A typical framework for FRS.}
    \label{fig:typical_FRS}
\end{figure}


\begin{definition}[Federated Recommendation System]
\label{def:frs}
A Federated Recommendation System is a technology that uses distributed algorithms for personalized information filtering. It aims to improve the accuracy of information filtering and the effectiveness of personalized services, while maintaining user privacy.
\end{definition}

FRSs enable collaborative learning across multiple clients (e.g., users or locations) without direct exchange of raw user data. 
Fig. \ref{fig:typical_FRS} illustrates that FRS typically involves three key processes: 1) client model update, 2) communication, and 3) global aggregation. 
Users train models locally using their own data and share updated parameters (e.g., gradients) with a server. 
The server then performs global aggregation, integrating information from all participants and redistributing updated parameters. 
This communication process preserves privacy and security.


% FRSs facilitate collaborative learning by pooling analysis and learning capabilities across multiple clients (e.g., users or locations), without the need for direct exchange of raw user data. 
% Fig. ref{fig:typical_FRS} illustrates that this type of system typically involves three processes: 1) client model update, 2) communication, and 3) global aggregation. 
% The client model update allows users to train their models locally on their devices using their own data and then upload the updated intermediate parameters, e.g., the model gradients or parameters can be shared, to the server. 
% The server then performs global aggregation on the parameters sent by all participants, integrating the unique information from each of them. 
% The aggregated parameters are then distributed to the next round of participants, initiating a new training round. 
% The process of uploading and distributing is collectively referred to as communication. 
% These approaches effectively preserve privacy and security.

% FRSs facilitate collaborative learning by pooling analysis and learning capabilities across multiple clients (e.g. users or locations), without the need for direct exchange of raw user data. 
% Fig. ref{fig:typical_FRS} illustrates that this type of system typically involves three processes: 1) client model update, 2) communication, and 3) global aggregation. 
% The client model update allows users to train their models locally on their devices using their own data and then upload the updated intermediate parameters, e.g. the model gradients or parameters can be shared, to the server. 
% The server then performs global aggregation on the parameters sent by all participants, integrating the unique information from each of them. The aggregated parameters are then distributed to the next round of participants, initiating a new training round. 
% The process of uploading and distributing is collectively referred to as communication.
% These approaches effectively preserves privacy and security. 

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.85\columnwidth]{figures/tax_fl.png}
    \caption{The diagram illustrates the taxonomy of FRS based on two main criteria: Data Distribution and Communication Architecture.}
    \label{fig:tax_frs}
\end{figure}


\subsubsection{Taxonomy of FRS}

\begin{figure*}[!hbp]
    \centering
    \subfloat[Horizontal FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_horizontal.png}
        \label{fig:horizontal_frs}
    }\hspace{10pt}
    \subfloat[Vertical FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_vertical.png}
        \label{fig:vertical_frs}
    }\hspace{10pt}
    \subfloat[Transfer FRS]{
        \includegraphics[width=.5\columnwidth]{figures/data_transfer.png}
        \label{fig:transfer_frs}
    }
    \caption{Typical data categories of FRS.}
    \label{fig:data_type}
\end{figure*}

As illustrated in Fig. \ref{fig:tax_frs}, FRSs can be categorized based on data distribution and communication architecture \cite{yang2020federated,sun2024survey}.

Based on data distribution, there are three types, each type addresses specific data collaboration and learning scenarios:
\begin{itemize}
    \item \textbf{Horizontal FRS} deals with situations where the feature spaces are similar across different entities, but the sample spaces differ, as shown in Fig. \ref{fig:horizontal_frs}. 
    For instance, two customers who shop at the same store may purchase some of the same products. 
    The horizontal method aggregates model updates from various sources to train recommendation models without sharing raw user data. This approach enhances the accuracy and efficiency of recommendation systems while safeguarding user privacy.
    Horizontal FRS is currently the most common type, with many studies~\cite{zhang2023dual,li2024federated,zhang2024federated} based on the assumption of this data distribution.
    
    \item \textbf{Vertical FRS} is applied when the feature spaces differ, but the sample spaces are similar, as shown in Fig. \ref{fig:vertical_frs}. 
    This scenario is common when different parties possess different types of data about the same users. 
    An example would be a bank and an online retailer holding distinct perspectives on the same customers, i.e., the bank has credit history while the retailer has shopping history. 
    One challenge is that how to align the identities of customers across different parties.
    Vertical FRS~\cite{zhang2021vertical,cao2023privacy,mai2023vertical,wan2023fedpdd}  trains recommendation models by securely integrating different data features between parties, utilizing richer user information for more accurate personalized recommendations and ensuring data privacy and security.
    
    \item \textbf{Transfer FRS} utilizes principles of transfer learning~\cite{zhuang2020comprehensive} to transfer knowledge from one domain to another, as shown in Fig. \ref{fig:transfer_frs}. This type is suited for scenarios with significant differences in both feature and sample spaces across parties. Transfer learning allows the system to leverage data and knowledge from the source domain to enhance recommendation performance in the target domain, even when the target domain lacks sufficient data for independent model training. Transfer FRS~\cite{zhang2024transfr} is particularly beneficial for emerging markets or user groups with limited data, drawing insights from related domains.
    
\end{itemize}


\begin{figure*}[!htbp]
    \centering
    \subfloat[Centralized FRS]{
        \label{fig:arch_cent}
        \includegraphics[width=.6\columnwidth]{figures/type_traditional.png}
    }\hspace{5pt}
    \subfloat[Semi-decentralized FRS]{
        \label{fig:arch_semi}
        \includegraphics[width=.6\columnwidth]{figures/type_semi-decentralized.png}
    }\hspace{5pt}
    \subfloat[Decentralized FRS]{
        \label{fig:arch_decent}
        \includegraphics[width=.6\columnwidth]{figures/type_decentralized.png}
    }
    \caption{Typical architecture categories of FRS.}
    \label{fig:archi_type}
\end{figure*}

As shown in Fig.~\ref{fig:archi_type}, FRS can be categorized into centralized, semi-decentralized and decentralized based on their communication architecture. Each type addresses privacy and scalability in different ways:
\begin{itemize}
    \item \textbf{Centralized FRS} operates within a FL framework where a central server orchestrates the learning process as shown in Fig. \ref{fig:arch_cent}. Clients locally compute updates based on their data and send these updates to the server. The server aggregates these updates to prompt essential information sharing, which is then distributed back to the users. 
    It effectively addresses privacy concerns by allowing the model to learn from decentralized data sources without centralizing the data itself.
    While this approach improves privacy by not requiring the sharing of raw data, it still relies on a central authority to manage the model. This architecture is typically used to overcome data silo issues~\cite{li2022federated} and improve the performance of RS without compromising user privacy and data security. Due to its simplicity and intuitive nature, this architecture has become the dominant framework within the field of FRS. There is a great deal of work \cite{zhang2023lightfr,zhang2023dual,li2024federated,zhang2024federated,zhang2024transfr} based on it currently.
    
    \item \textbf{Semi-decentralized FRS} shown in Fig. \ref{fig:arch_semi} introduces an intermediate layer between the central server and the users, such as edge servers or devices that can perform additional computational or storage tasks. This setup aims to reduce the communication overhead and latency associated with sending updates to a central server, especially in large-scale applications. 
    A specific example is the SemiDFEGL framework~\cite{qu2023semi}, which improves scalability and reduces communication costs by introducing new device-to-device collaborations. 
    It augments local subgraphs with predicted interacted item nodes to exploit high-order collaborative information between users and items in a privacy-preserving manner, which is particularly useful for recommendations based on collaborative filtering and graph neural networks.
    
    \item \textbf{Decentralized FRS}, which employs peer-to-peer communication architecture~\cite{hegedHus2019decentralized}, distributes the learning process completely to all participating devices, without the need for a central server for model aggregation, as shown in Fig. \ref{fig:arch_decent}. 
    This approach maximizes privacy and data ownership, but presents challenges in coordinating model updates and ensuring model convergence. 
    Zheng et al.~\cite{zheng2023decentralized} proposed a FRS model called DGREC by adopting a decentralized graph neural network, which constructs a local intra-item hypergraph and a global inter-user graph for each user, allowing users to freely choose whether to disclose their interactions. Li et al.~\cite{li2024decentralized} introduced DFedRec, which uses a privacy-aware client-level structured graph to share model parameters only with relevant neighboring users, thereby reducing communication costs and protecting user privacy.
\end{itemize}
Each of these architectures offers a trade-off between privacy, communication efficiency and the degree of decentralization. 
Centralized systems simplify model aggregation, but rely on a central authority. 
Semi-decentralized systems aim to balance efficiency and privacy with an intermediate layer, while decentralized systems offer the highest level of privacy at the cost of more complex model coordination.


% \begin{figure}[!htbp]
%     \centering
%     \subfloat[VAE]{
%         \label{fig:gen_vae}
%         \includegraphics[height=3.7cm]{figures/gen_vae.png}
%     }\hspace{1pt}
%     \subfloat[GAN]{
%         \label{fig:gen_gan}
%         \includegraphics[height=3.7cm]{figures/gen_gan.png}
%     }\hspace{1pt}
%     \subfloat[DM]{
%         \label{fig:gen_dm}
%         \includegraphics[height=3.7cm]{figures/gen_dm.png}
%     }\hspace{1pt}
%     \subfloat[LLM]{
%         \label{fig:gen_llm}
%         \includegraphics[height=3.7cm]{figures/gen_llm.png}
%     }
%     \caption{Architectural Comparison of Foundation Models: VAE, GAN, DM, and LLM.}
%     \label{fig:gen_type}
% \end{figure}


\subsection{Foundation Model}

The rapid increase in the performance of computer hardwares, e.g., GPUs, the increasing maturity of transformer architectures, and the public availability of large amounts of training data have been three key factors in the emergence of FM~\cite{bommasani2021opportunities}. 
According to the work of Stanford HAI~\cite{bommasani2021opportunities}, we have the following definition of FM:
\begin{definition}[Foundation Model]
\label{def:fm}
    A foundation model is defined as any model trained on extensive data (typically using large-scale self-supervised learning) that is capable of adapting to a wide range of downstream tasks, for instance, through fine-tuning or prompting.
\end{definition}

In recent years, the scale and scope of FM have greatly expanded our imagination of potential applications. 
Such models typically have billions or even trillions of parameters, allowing them to learn more complex patterns and knowledge. They can be adapted to new tasks through fine-tuning or prompting~\cite{church2021emerging,yuan2023power}. 
For instance, the GPT-3 model~\cite{brown2020language}, comprising 175 billion parameters, is capable of adapting and perform various tasks with the aid of natural language prompts, despite the fact that a significant proportion of these tasks have not been explicitly trained.

FM is distinguished by two key characteristics~\cite{bommasani2021opportunities}: 1) \textit{Emergence}, which refers to the implicit induction of system behavior from examples, as opposed to explicit design; and 2) \textit{Homogenization}, which indicates that the method of constructing machine learning systems tends to be unified across a wide range of applications. 
Although FM is based on self-supervised learning and transfer learning, their scale brings new emergent abilities, and their effectiveness in many tasks has motivated homogenization, e.g., many FMs have evolved based on transformer architectures~\cite{devlin2018bert,liu2019roberta,dosovitskiy2020image,brown2020language}. While homogenization provides strong leverage, it also requires caution, as defects in foundation models can be inherited by all downstream adapted models. Despite the broad deployment prospects of foundation models, due to their emergent properties, our understanding of how they work, when they fail, and what they can actually do is still quite limited~\cite{bommasani2021opportunities}, but there has been quite a bit of work~\cite{wei2022chain,yang2024foundation,zhao2024explainability} that attempts to explain this phenomenon.
Moreover, OpenAI proposes a Scaling Law for LLM~\cite{kaplan2020scaling}, suggesting that the performance of a model is governed by a power-law relationship involving computational power, model parameters, and data size. This law also applies to downstream tasks~\cite{isik2024scaling}. Therefore, understanding and leveraging this power-law relationship when using FM can aid in more efficiently allocating resources and optimizing model performance.

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.85\columnwidth]{figures/tax_fm.png}
    \caption{The diagram illustrates the taxonomy of FM based on two main criteria: Data Type and Functionality.}
    \label{fig:tax_fm}
\end{figure}

\subsubsection{Taxonomy of FM}
As shown in Fig. \ref{fig:tax_fm}, similar to FRS, FM can also be classified based on data type or functionality. 
Specifically, based on the type of data used during training, FM is mainly divided into followings \cite{bommasani2021opportunities}:
\begin{itemize}
    \item \textbf{Language FM}: These types of FM mainly deal with textual data and are trained on large textual datasets to understand and generate language~\cite{devlin2018bert,liu2019roberta}. 
    They are very effective in natural language processing (NLP) tasks such as machine translation \cite{dabre2020survey}, search \cite{lu2020twinbert,liu2021pre}, and sentiment analysis \cite{mathew2020review}. Typical language models include BERT \cite{devlin2018bert}, GPT-3 \cite{brown2020language}, and LLama \cite{touvron2023llama}, which typically use deep transformer architectures that are able to capture complex linguistic regularities and demonstrate excellent performance on multilingual tasks.
    \item \textbf{Vision FM}: Vision FM focuses on processing and understanding image data. These models are able to perform tasks such as object recognition \cite{dosovitskiy2020image,wang2023all,zhang2023recognize}, image segmentation \cite{kirillov2023segment,wang2023seggpt,zou2024segment}, and visual reasoning \cite{huang2022perceive,ding2023visual} by learning large amounts of image data. For example, DINOv2 \cite{oquab2023dinov2} and SAM \cite{kirillov2023segment} are basic models trained specifically for visual tasks, and using self-supervised learning methods, these models learn valid visual representations without labelling the data.
    \item \textbf{Multi-modal FM}: Multi-modal models can simultaneously process and understand multiple types of data, such as text and images. Such models can excel in cross-modal tasks such as image captioning and visual quizzing \cite{bai2023qwen,wang2023cogvlm,you2023ferret} by integrating information from different modalities. CLIP \cite{radford2021learning} and DALL·E \cite{tamkin2021understanding} are representative of such models that are able to understand the relationship between an image and its corresponding textual descriptions, demonstrating flexibility and robustness in handling multiple data types.
\end{itemize}

Functionally, FMs are generally categorized into two types \cite{bommasani2021opportunities,liu2023towards,wu2023survey}:
\begin{itemize}
    \item \textbf{Discriminative FM}: The main task of discriminative FM is to distinguish or predict specific outputs from given input data. These models are generally based on the BERT family and are more concerned with learning decision boundaries from the data to perform tasks like classification \cite{yao2022prompt,chen2023robust} and regression \cite{ali2023evaluating}.
    \item \textbf{Generative FM}: The core goal of generative FM is to learn the distribution of the data and be able to generate new data samples \cite{cao2023comprehensive}. These models, such as GPT-3, DALL·E, etc., are able to capture the underlying structure of the data and thus generate new instances that are similar but different from the training data. Generative FM has a wide range of applications in areas such as the generation  of text \cite{otter2020survey} and images \cite{ho2022cascaded,saharia2022palette}.
\end{itemize}

\subsubsection{Adaptation}

Fig.~\ref{fig:fm} illustrates a commonly used technique for pre-trained models, known as the Adaptation. 
This technique adds new lightweight layers while maintaining the original parameters of the pre-trained model, enabling fine-tuning and extension for specific tasks \cite{ding2023parameter,zhang2024federated}. 
This approach is suitable for multi-task learning and tasks performed in resource-limited environments, such as few-shot learning \cite{liu2024few}. 
Adaptations have found wide applications in natural language processing  and computer vision tasks \cite{hu2021lora,dettmers2024qlora,gao2024clip} .
%%% 插入大量文献
According to \cite{liu2024few}, adaptation methods are categorized into three main types:
\begin{itemize}
    \item \textbf{Prompt-based Fine-tuning Adaptation Methods} are inspired by the principles of prompt learning in NLP, adapts the model to a specific downstream task by using a portion of the fixed text input as a learnable vector and fine-tuning it using downstream task data. For instance, CoOp~\cite{zhou2022learning} introduces the concept of prompt learning into the adaptation of downstream tasks for multimodal pre-trained foundation models by automatically constructing contextual prompts using learnable word embeddings. CoCoOp~\cite{zhou2022conditional} builds upon this by creating a meta-network that learns image features, which are then combined with prompt vectors to enhance the generalization performance of CoOp on new category data.

    \item \textbf{Adapter-based Fine-tuning Adaptation Methods} entail the incorporation of small, trainable modules called Adapters into a pre-trained model. These adapters are subjected to fine-tuning, rather than the entire model, thereby enabling the model to adapt to novel tasks with minimal alterations to its original parameters. CLIP-Adapter \cite{gao2024clip} adds simple adapter structures within the CLIP model that are fine-tuned using a small dataset. This method allows the model to adapt to new tasks by learning task-specific features without the need for extensive retraining of the entire model. CALIP \cite{guo2023calip} enhances the cross-modal interaction capabilities of adapters by integrating text and image features using attention maps and incorporating two trainable linear layers before and after this integration. LoRA \cite{hu2021lora} adjusts the weights of a pre-trained model by multiplying the weight matrices with a low-rank matrix, allowing for fine-tuning of the model without significantly increasing the number of parameters. 

    \item \textbf{External Knowledge-based Adaptation Methods} integrate external knowledge (e.g., from knowledge graphs or additional language model queries) into the adaptation process. This is particularly advantageous for enhancing the model's comprehension and efficacy in tasks where domain-specific knowledge is vital but data is scarce.  CuPL \cite{pratt2023does}enhances zero-shot classification performance by asking questions to a LLM and generating multiple descriptive statements for each category, enriching the semantics of the categories. LaBo \cite{yang2023language} uses GPT-3 to generate a large pool of candidate feature descriptors. It then selects the optimal subset of descriptors for classification decisions, considering the distinctiveness of features for other categories and the coverage for the current category.

\end{itemize}










==> TKDE/sections/sec_bio.tex <==
%!TEX root = ../main.tex

% \begin{IEEEbiographynophoto}{Zhiwei Li}
% Biography text here without a photo.
% \end{IEEEbiographynophoto}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/zhwl.jpg}}]{Zhiwei Li}
is pursuing his PhD at University of Technology Sydney. 
His research focuses on advancing personalized federated collaborative filtering by developing models that improve recommendation accuracy while ensuring user privacy. 
He has authored several influential papers, contributing to key areas of federated recommendation, including personalized item representations, multimodal data integration, and the application of foundation models in federated settings. 
He also serves as a reviewer for leading conferences, demonstrating his expertise.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/gdl1.jpg}}]{Guodong Long}
is a leading scholar in AI, and serves as Co-Director of the Representation Learning for Machine Intelligence Lab at University of Technology Sydney. 
His research focuses on trustworthy AI, personalized intelligence in federated learning, and on-device intelligence integrated with foundation models.
He has published about 150 papers, with over 24,000 citations (h-index: 50), featuring in top conferences like NeurIPS, ICML, and ICLR. 
In 2024, he ranked 21st globally in the AAAI/IJCAI domain on the AI 2000 Most Influential Scholars list.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/chxzh.jpg}}]{Chunxu Zhang}
completed her Doctoral degree at Jilin University, working on federated learning and recommender systems. 
She has published over 20 papers in top-tier venues (e.g., WWW, KDD, SIGIR, IJCAI, AAAI, and NeurIPS). 
In addition, she has been invited to be a reviewer for numerous distinguished conferences and journals such as WWW, KDD, ICLR, IJCAI, TNNLS, and TIFS.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/hlzh.jpg}}]{Honglei Zhang}
is currently pursuing his Ph.D. at Beijing Jiaotong University. 
During this period, he was a visiting scholar at Nanyang Technological University. 
His research work has been published on top-tier international venues, including ICDE, TOIS, and TNNLS. Additionally, he has been an PC and/or reviewer for many leading venues, such as WWW, NeurIPS, ICLR, TKDE and TOIS. 
His research interest primarily focuses on developing efficient and privacy-preserving recommender systems, with a particular interest in federated recommendation.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/jj1.jpg}}]{Jing Jiang}
is an ARC DECRA Fellow and an Associate Professor in the School of Computer Science and a core member of the Australian Artificial Intelligence Institute at University of Technology Sydney. 
Her research focuses on machine learning and its applications, with over 80 publications in top AI conferences and journals such as NeurIPS, ICML, ICLR, and IEEE TPAMI. 
Prof. Jiang has served as a program committee member for leading AI conferences and a reviewer for prestigious journals.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/chqzh.jpg}}]{Chengqi Zhang}
is a leading expert in Distributed Artificial Intelligence and Data Mining, with over 388 publications and 34,500+ citations (H-index: 71)
As the founding Director of UTS’s Quantum Computation and Intelligent Systems Centre, he secured AU\$16.9 million in funding, establishing it as Australia’s top IT research hub and elevating UTS computer science into the global top 100 rankings.
His global influence is reflected in keynote talks at 33 major conferences and leadership roles, and His contributions have earned prestigious awards.
\end{IEEEbiography}


==> TKDE/sections/sec_challenges.tex <==
%!TEX root = ../main.tex

\section{Key Challenges and Strategic Solutions}
\label{sec:challenge}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/challenges.pdf}
    \caption{
        Challenges in integrating FMs into FRSs, divided into data and model challenges, highlighting areas requiring strategic solutions for enhanced personalization and privacy.
        }
    \label{fig:chal}
 \end{figure}   

Integrating FMs into FRSs has introduced new opportunities for enhancing personalized recommendations while maintaining user privacy. 
However, as illustrated in Fig. \ref{fig:chal}, this integration presents significant challenges across multiple dimensions. 
Understanding these challenges comprehensively and developing effective strategies to address them is crucial for advancing FRSs. 
This section explores these challenges in depth and presents potential strategies to overcome them.


\subsection{Data Challenges and Mitigation Strategies}

\subsubsection{Privacy Concerns}
Privacy aims to prevent unauthorized access or misuse of data, especially during model training and data handling, to protect user identities and personal details \cite{hasan2023security}. 
In a federated setting, safeguarding user privacy is of utmost importance. 
Privacy concerns focus on preventing unintended exposure or misuse of personal data, ensuring that sensitive information remains confidential. 
While training and recommendations must occur without revealing personal data, FMs, such as GPT-3, may memorize and reproduce training data, potentially leaking sensitive information \cite{chen2023hide}. 
Additionally, if generated data closely resembles original data, user privacy risks may arise \cite{hasan2023security}.

To mitigate these privacy concerns, differential privacy \cite{minto2021stronger} can be employed by adding noise during model training to reduce data leakage risks while preserving model performance. 
Homomorphic encryption \cite{acar2018survey} allows training on encrypted data, effectively preventing data theft during transmission and processing. 
Moreover, machine unlearning techniques \cite{bourtoule2021machine} can be utilized to remove specific user data from the FMs, ensuring compliance with privacy regulations like GDPR.
An emerging approach, known as privacy rewrite, transforms sensitive data into anonymized formats before transmission. Frameworks like HaS \cite{chen2023hide} exemplify this by anonymizing private entities locally and reconstructing them after processing. This method reduces privacy risks, preserves data utility, and minimizes computational overhead. 

\subsubsection{Security Threats}
Security threats involve protecting data from malicious attacks or breaches \cite{hasan2023security}. 
While privacy controls who can access and use data, security emphasizes maintaining data integrity and defending against threats such as cyberattacks \cite{nasr2019comprehensive}. 
The integration of FMs into FRSs also necessitates ensuring data security, as participants may be subject to attacks like Member Inference Attacks \cite{nasr2019comprehensive}, Data Reconstruction Attacks \cite{lyu2021novel}, and Poisoning Attacks \cite{tolpegin2020data}, which can compromise model integrity or data quality.

To ensure data integrity and confidentiality during transmission, secure multi-party computation \cite{byrd2020differentially} can distribute computational tasks among multiple participants, preventing any single party from accessing complete data. Additionally, blockchain \cite{hai2022bvflemr,guo2023decentralized} can record data access and operations, enhancing data integrity, traceability, and transparency.

\subsubsection{Data Scarcity}
Despite FMs' potential to alleviate data sparsity, FRSs often face data scarcity, especially in scenarios where participants have limited interaction data under federated Settings \cite{alamgir2022federated}. 
Data sparsity can significantly impact model performance, particularly when user interactions are insufficient to build effective models.

Data augmentation techniques \cite{van2001art,mumuni2022data} can be used to generate diverse training samples, expanding the dataset size. Knowledge transfer \cite{chen2024percept} from rich datasets in other domains can also alleviate data sparsity, improving overall model performance. When employing generative FMs \cite{waqas2023revolutionizing,rossi2024augmenting}, quality control mechanisms are essential to ensure that synthetic data meets quality standards without introducing biases.

\subsubsection{Data Imbalance}
In federated settings, significant differences in data size and distribution exist across clients, causing data imbalance \cite{duan2020self,wang2021addressing,luo2022towards}. 
This imbalance, often driven by long-tail distributions of item labels and user behaviors, affects model training effectiveness.

To address sample imbalance, resampling techniques like oversampling minority classes or undersampling majority classes \cite{he2009learning} can be used. 
Weighted loss functions \cite{li2021autobalance,duan2020self} can also be used to assign higher importance to minority class samples during training, improving the capability to recognize underrepresented data without altering the data distribution.

\subsection{Model Challenges and Strategic Solutions}

\subsubsection{Synchronization Overhead}
In federated settings, the need for frequent synchronization between participants and the central server can result in high communication costs and system complexity, especially when dealing with large FMs with extensive parameters \cite{bommasani2021opportunities}.

Gradient compression \cite{lin2017deep} can help reduce the data transmitted during synchronization, thereby lowering communication costs. 
Asynchronous update strategies \cite{chen2019communication} that allow participants to update models independently, followed by periodic global synchronization, also enhance system efficiency.

\subsubsection{Client Heterogeneity}
Arising from variations in model types, sizes, and architectures, this issue creates challenges when deploying a unified FM in federated settings \cite{zhu2018knowledge}.

Adaptive training algorithms \cite{tian2019contrastive,zhang2021parameterized} that adjust model parameters based on each client's computational capabilities and data characteristics can address this issue. Knowledge transfer \cite{zhang2024transfr} between clients can further enhance model performance by mitigating disparities.

\subsubsection{Interpretability and Transparency}
FMs are often perceived as black-box models, which makes it challenging to understand their internal workings and may lead to issues with trust and compliance \cite{ren2024advances}.

Explainable AI \cite{gunning2019xai}, such as attention mechanisms \cite{mohankumar2020towards} and feature importance analysis \cite{carletti2019explainable}, offer insights into model decisions, enhancing transparency. 
Additionally, generative FMs \cite{schneider2024explainable} generate natural language explanations for recommendations, fostering user trust and acceptance.


















==> TKDE/sections/sec_conclusion.tex <==
%!TEX root = ../main.tex

\section{Conclusion}
\label{sec:conclusion}

This paper comprehensively examines the integration of FRSs with FMs, a direction that has gained attention for its ability to protect user privacy. 
It begins by summarizing common approaches of FRSs and FMs, then delves into the challenges faced during integration. 
To address these challenges, we comprehensively various strategies to adapt to data diversity, employing privacy-preserving methods, and reducing communication overhead through model compression and efficient communication protocols.

This work also discusses the future research directions directions indicating that FRSs can provide more accurate personalized recommendations while better protecting user privacy. 
Additionally, we showcase applications of FRS in various fields, demonstrating their potential and value in the real world. 
Through this paper, we aim to provide a guidance for integrating FRS with FM, directing future research and technological advancements to collectively advance this field.

% The survey concludes that FRS enhanced by FM hold great promise for overcoming challenges such as data sparsity and privacy concerns. 
% By exploiting the generative capabilities of GMs such as DMs and LLMs, these systems can better mimic the underlying data distributions, potentially improving recommendation accuracy while preserving user privacy. 
% The integration of GMs into FRS represents a fertile ground for future research, promising advances in both theoretical understanding and practical applications. 
% This review aims to stimulate further exploration and development in this innovative and important area, encouraging researchers to address the challenges identified and explore the future directions outlined.

==> TKDE/sections/sec_dir.tex <==
%!TEX root = ../main.tex


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/dir.pdf}
    \caption{
        Key future directions for integrating FMs into FRSs aim to address emerging challenges and opportunities, focusing on enhancing recommendation performance, safeguarding user privacy, and improving system adaptability.
        }
    \label{fig:dir}
 \end{figure}   

\section{Future Directions}
\label{sec:dir}

The emerging field of applying FMs to FRSs presents both opportunities and challenges, shown in Fig. \ref{fig:dir}. 
By leveraging the powerful representation capabilities of FMs and the privacy-preserving advantages of FRSs, it is possible to significantly enhance recommendation performance while addressing some of the long-standing challenges faced by traditional methods. 
This section discusses several key future directions for integrating FMs into FRSs, focusing on specific problems, FMs' advantages, the new challenges introduced, and potential research directions. 
Sec. \ref{sec:dir} aims to guide future research and applications towards delivering higher-quality recommendation services while protecting user privacy.

\subsection{Data Augmentation}
The challenge of data scarcity is a common problem in FRS due to data privacy constraints. Generative FMs, such as Large Language Models (LLMs) and Diffusion Models (DMs), can be utilized to alleviate this issue by generating synthetic user interaction data for training purposes, which can help mitigate data imbalance and scarcity \cite{feng2021survey,yang2022image}. FM can generate virtual interaction records or additional item descriptions, thereby enhancing user profiles and improving recommendation accuracy and personalization \cite{yan2019differentiated}.

However, the use of generated data introduces challenges related to data quality and potential biases, which may degrade the performance of recommendation systems. Rigorous validation and cleaning are necessary to ensure that the synthetic data is statistically consistent with real data, thereby reducing noise and biases \cite{maharana2022review}. Furthermore, integrating privacy-preserving techniques, such as differential privacy, can ensure that synthetic data generation does not reveal sensitive user information. Research should also focus on generating diverse data to cover a wide range of scenarios and user behaviors, thus reducing the risks of bias and overfitting \cite{li2019insufficient}.

\subsection{Cold-Start Recommendation}
The cold-start problem, caused by a lack of sufficient historical interaction data for new users or items, presents a significant challenge for FRSs \cite{schein2002methods}. FMs, pre-trained on large amounts of textual data, possesses rich semantic knowledge that can be leveraged for generating high-quality representations of users and items, enabling zero-shot and few-shot learning to address cold-start scenarios \cite{gong2023unified,zhang2024federated}.

Despite FMs' capabilities, ensuring user privacy in a federated environment remains challenging. Additionally, multi-task learning techniques can be explored to improve model adaptability and generalization across different domains, allowing the model to provide effective recommendations for new users and items while maintaining privacy \cite{yu2024unleashing}. Future research should focus on enhancing privacy-preserving mechanisms and exploring efficient knowledge transfer techniques to support cold-start recommendations.

\subsection{Multi-Modal Recommendation}
The ability to process and integrate different modalities of data, such as text, images, audio, and video, is one of FM's key strengths \cite{bommasani2021opportunities}. By incorporating multi-modal data, FM can construct more comprehensive user profiles  \cite{li2024personalized}, which in turn enhances the personalization of recommendation services \cite{geng2023personalized,huang2024foundation}. This richer profiling allows for more accurate user interest representation and better recommendation quality.

However, the heterogeneity of multi-modal data poses a challenge, as different data modalities have distinct structures and characteristics \cite{wang2021survey}. Developing unified representation methods to map different modalities into a common space is crucial for seamless model integration \cite{li2024personalized}. Privacy is also a concern, as multi-modal data often contains more sensitive information \cite{feng2024robust,wu2024towards}. Future research should focus on developing robust privacy-preserving techniques tailored for multi-modal data and improving computational efficiency in processing and integrating these diverse data types.

\subsection{Real-Time Recommendations}
Real-time recommendation is critical in FRS, as it allows for dynamically adapting recommendations based on real-time user behavior and contextual data \cite{huang2015tencentrec}. FM's contextual understanding capabilities enhance the accuracy and relevance of real-time recommendations by effectively processing user queries and item descriptions.

However, real-time recommendations require extremely low latency, which places a high demand on computational resources. FM's high computational requirements may introduce latency issues, adversely affecting the user experience. Future research should focus on model compression and acceleration techniques, such as distillation \cite{kang2022personalized} and pruning \cite{beel2019data}, to reduce computational complexity and improve response times. Additionally, methods like sliding windows can be used to manage the input context efficiently, optimizing the handling of long sequences of user behavior.

\subsection{Enhanced Explainability}
Explainability is an essential aspect of FRS, as providing transparent explanations for recommendations increases user trust and satisfaction. Language FMs, pre-trained on extensive text data, are capable of generating coherent and informative explanations that can help users understand the reasons behind recommendations \cite{hada2021rexplug,geng2022path}. For example, models such as ChatGPT can generate natural language explanations for why specific items are recommended \cite{liu2023chatgpt}.

The challenge, however, lies in the computational cost associated with generating these detailed explanations, especially for large language models, which can lead to latency issues \cite{bommasani2021opportunities}. 
Moreover, biases present in pre-training data may lead to unfair or biased explanations \cite{zhuang2023foundation}. 
Future research should focus on model compression to reduce computational costs and on debiasing methods to minimize biases in generated explanations. 
Incorporating user feedback may further help improve the quality and fairness of recommendation explanations.

\subsection{Advanced Metrics}
The evaluation of FRSs with FMs requires advanced metrics that extend beyond traditional metrics like rating prediction or item ranking \cite{xu2024survey}. 
Given FM's ability to generate new items and provide explanations, traditional metrics may not fully capture its performance. 
New evaluation metrics that account for the generative and explanatory capabilities of FMs are needed to better assess recommendation quality in these emerging scenarios \cite{wu2023survey}.

Future research should explore comprehensive evaluation criteria that consider aspects such as diversity, fairness, and user satisfaction to provide a holistic assessment of FRS performance with FM integration.


==> TKDE/sections/sec_intro.tex <==
%!TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

In the digital age, the exponential growth of information has created a need for systems that navigate, filter, and personalize data for individual users. 
Recommendation Systems (RS) have become crucial tools for filtering online information and helping users discover products, content, and services that align with their preferences~\cite{ko2022survey}. 
However, these systems traditionally rely heavily on centralized data collection and processing, posing significant privacy risks and operational bottlenecks.
%
User privacy has become increasingly important, especially with stringent data protection regulations such as the General Data Protection Regulation (GDPR)~\cite{voigt2017eu}, emphasizing storing user data locally rather than uploading it to servers.

To address these privacy concerns, Google introduced Federated Learning (FL)~\cite{mcmahan2017communication}, designed to train models across distributed devices while keeping data localized. 
This paradigm shift in data processing leverages the computational capabilities of individual devices for local data analysis. 
Specifically, FL alternates between training models locally on each client and aggregating parameters globally on a central server.
%
The integration of FL with RS is essential for safeguarding user privacy in recommendation services, giving rise to the burgeoning field of Federated Recommendation Systems (FRSs)~\cite{zhang2021survey}. 

FRSs have shown promising results in various areas, such as service provision~\cite{yuan2022privacy,yin2022fgc}, daily scheduling~\cite{huang2021feddsr}, and driving planning~\cite{lu2021fmfparking,vyas2023federated}, impacting multiple facets of daily life.  
However, in most cases, each client typically consists of a single user's device, containing only the data of one user's accessed items, which is extremely small compared to the total item set, creating a serious data scarcity problem. 
In addition, different users have different behaviors and preferences, leading to significant data heterogeneity. 
The presence of both issues can result in sub-optimal models and reduced effectiveness.
Addressing these challenges is crucial for the success of FRSs, particularly as they become more widely adopted in privacy-sensitive domains. Innovative strategies to enhance data sharing and model personalization while maintaining privacy are needed to overcome data scarcity and heterogeneity.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/FM.pdf}
    \caption{The foundation model can integrate information contained in data from various modalities during pre-training. The model can then be adapted for a variety of downstream tasks through adapters such as prompting or fine-tuning.}
    \label{fig:fm}
\end{figure}

More recently, a novel paradigm for constructing artificial intelligence (AI) systems, known as Foundation Models (FMs) \cite{bommasani2021opportunities} (or Pretrained Large Models  \cite{han2021pre}), has garnered considerable interest following the remarkable success of models like ChatGPT \cite{openai2022chatgpt} and various diffusion models \cite{ho2020denoising,ho2022cascaded,saharia2022palette}.
As illustrated in Fig.~\ref{fig:fm}, this paradigm involves using self-supervised learning objectives to pre-train models on large amounts of unlabeled data. 
This process, referred to as Pre-Training, enables the models to learn general-purpose representations.
Once pre-trained, FMs can be adapted to specific tasks through techniques such as \textbf{Fine-Tuning} \cite{zhang2024scaling} or \textbf{Prompting} \cite{gu2023systematic}, turning the general model into a task-specific one. 
This adaptability allows FMs to achieve state-of-the-art performance across a wide range of applications.
Examples of FMs include language models like BERT~\cite{devlin2018bert} and vision models like ViT~\cite{dosovitskiy2020image}, which have significantly advanced natural language understanding and computer vision, respectively. Multi-modal models like CLIP~\cite{radford2021learning} and DALL·E~\cite{tamkin2021understanding} extend these capabilities to handle both text and images, enabling tasks such as image-text retrieval and text-to-image generation.

The widespread adoption and success of FMs demonstrate their profound impact on AI research and applications. 
% In this paper, we focus on exploring the potential of FMs in the context of FRSs, discussing how their generalization capabilities and adaptability can address existing challenges and pave the way for future advancements.
FMs are typically trained on substantial quantities of data from diverse sources, enabling them to incorporate extensive knowledge when tackling specific downstream tasks \cite{bommasani2021opportunities}. 
This characteristic offers several significant benefits for FRSs \cite{zhang2024transfr}: 
Firstly, FMs can alleviate the data sparsity issue by providing rich pre-trained representations, thus enhancing recommendation accuracy even with limited user interactions. 
Secondly, they effectively mitigate the cold-start problem for new users and items by leveraging learned general patterns. 
Thirdly, FMs facilitate efficient transfer learning, allowing models to adapt quickly to new domains or tasks with minimal additional training.
Moreover, the use of FMs can help balance privacy and performance; their pre-trained capabilities reduce the need for extensive data sharing and multiple rounds of communication in federated settings, thereby lowering the computational and communication costs associated with federated training.
Given these considerable advantages, integrating FMs into FRSs is not just a viable approach but a necessary progression to overcome existing limitations and drive innovation in the field.

Although integrating FMs into FRSs holds immense promise, it must be acknowledged that this field is still in its nascent stages, with an insufficient understanding of the challenges, viable methods, and directions for development. 
This paper aims to bridge this knowledge gap through an in-depth analysis of the integration of FMs and FRSs. 
We provide a comprehensive examination of the motivations and challenges associated with uniting these two paradigms, drawing on insights from recent studies, which highlight the benefits of introducing FMs in federated recommendation scenarios. 
Additionally, we outline future development trends and potential applications. 
By elucidating the intersection of FRSs and FMs, this paper aims to promote further exploration and innovation within this emerging field, thereby facilitating its rapid advancement.
The paper also emphasizes the critical role of pre-trained representations in addressing challenges like data sparsity and heterogeneity, which are inherent in FRSs.

% the emergence of a novel paradigm for the construction of artificial intelligence (AI) systems has garnered considerable interest in the wake of the remarkable success of ChatGPT~\cite{openai2022chatgpt} and diffusion models~\cite{ho2020denoising,ho2022cascaded,saharia2022palette} in the tasks of language understanding \cite{savinov2021step,li2022diffusion,gao2023exploring,ma2023large} and image generation~\cite{ho2022cascaded,saharia2022palette}, which we refer to as Foundation Models (FM)~\cite{bommasani2021opportunities}. 
% As shown in Fig. ref{fig:fm}, this paradigm is built by using self-supervised optimization objective to determine how to update model parameters based on model predictions on a large amount of unlabeled training data. This process is referred to as Pre-Training.
% Then, FM can utilize a technique, called Adaptation, to turn the general FM into a task-specific one. This process is termed as Fine-tuning or Prompting.
% Language models, e.g. BERT \cite{devlin2018bert} and RoBERTa \cite{liu2019roberta}, are usually trained using the next token prediction goal, which refers to the extent to which the model is able to predict the next token in the sequence.
% One of the most successful examples of language models is ChatGPT, which is based on GPT-3.5. By training on large amounts of text data, it aligns the capabilities of large language models (LLM) with human intent \cite{bommasani2021opportunities}.
% Vision models like ViT \cite{dosovitskiy2020image} are typically trained using either contrastive learning or diffusion training targets. 
% For contrastive learning \cite{wang2024generated}, images are randomly augmented before evaluating the similarity of the model representations. 
% For diffusion models \cite{ho2020denoising,ho2022cascaded,saharia2022palette}, noise is added to the images and the model is gradually de-noised by the target. 
% There are also multi-modal training targets, some of which separate images and text during training, while others consider both. 
% The foundation model, once trained, is used as a plug-in in combination with adaptations to achieve results for a wide variety of downstream tasks. 
% CLIP \cite{radford2021learning} and DALL·E \cite{tamkin2021understanding} are two multi-modal AI models developed by OpenAI. CLIP focuses on understanding images through natural language, while DALL·E focuses on generating images based on text descriptions. While both models are trained on large datasets of images and text, CLIP is primarily used for image retrieval and classification, while DALL·E excels at generating new images that match text descriptions \cite{cao2023comprehensive}.

% As FM is frequently trained using a substantial quantity of data from multiple sources, they are capable of incorporating a considerable amount of additional knowledge when performing a specific downstream task. This feature enables FM to provide diverse training data for task-specific models in downstream task scenarios, thus effectively alleviating the problem of data scarcity. Given these considerations, the application of FM to FRSs is not only a viable approach but also holds significant research potential. Such integration will drive innovation in FRSs.

% Although the application of FM to FRSs has the potential to be highly beneficial, it must be acknowledged that this field is still in its nascent stages, with an insufficient understanding of the challenges, viable methods, and directions for development. This paper aims to bridge this knowledge gap through an in-depth analysis of the integration of FM and FRSs. 
% The article provides a comprehensive examination of the motivations and challenges associated with integrating these two paradigms, with a particular focus on several representative technologies. Additionally, we outline future development trends and their applications. By elucidating the intersection of FRSs and FM, this study aims to promote further exploration and innovation within this emerging field, thereby facilitating its rapid advancement.


\textbf{Paper Organization.}
The reminder is structured to provide a thorough study of the current research landscape, technical challenges, application cases, and future directions of FRSs. 
The organization is as follows:
Sec. \ref{sec:related} outlines the existing surveys within the field of FRSs, and distinctly highlights our novel contributions, setting our paper apart from the current literature.
Sec. \ref{sec:bg} introduce foundational knowledge in the field of FRSs and FM, including definitions, basic architectures, and current scenario taxonomy.
Sec. \ref{sec:frs_w_fm} introduces the potential applications and functions of FM according to the three classical phases of FRSs.
Sec. \ref{sec:res} summarizes the datasets and evaluation methods commonly used in FRSs with FM, explaining how to quantify the recommendation performances.
Sec. \ref{sec:challenge} delves into the main technical challenges faced by FRSs with FM, including data heterogeneity, model aggregation difficulties, and privacy concerns, as well as current methods and their limitations in addressing these challenges.
Sec. \ref{sec:dir} explores future research directions in FRSs, including unresolved issues and emerging research areas, providing guidance and inspiration for researchers in the field.
Sec. \ref{sec:conclusion} concludes our paper with a summary of key findings and perspectives, offering insights into the trends and potential future of FRSs.



==> TKDE/sections/sec_related.tex <==
%!TEX root = ../main.tex

\section{Related Surveys and Contribution}
\label{sec:related}

In the field of FRSs, several surveys have been conducted to synthesize methodologies, privacy preservation techniques, and inherent challenges, each emphasizing different aspects.
Yang et al.~\cite{yang2020federated} discuss the practical implementation and evaluation of FRSs, focusing on system architecture and algorithmic efficiency.
Alamgir et al.~\cite{alamgir2022federated} provide a comprehensive overview of FRSs, highlighting techniques, prevailing challenges, and future directions.
Javeed et al.~\cite{javeedFederatedLearningbasedPersonalized2024} focus on security and privacy concerns in personalized RSs, proposing targeted solutions to these challenges.
Finally, Sun et al.~\cite{sun2024survey} conduct a survey comparing existing federated recommendation research, highlighting the strengths and limitations of various approaches.
Collectively, these surveys emphasize the critical importance of privacy protection and address challenges posed by data heterogeneity and model aggregation in FRSs. This work enhances our understanding of FRSs and provides a foundation for future research to tackle challenges.

While several studies have explored the combination of FMs with FL \cite{chen2023federated,zhuang2023foundation,yu2023federated,woisetschlager2024survey,chen2023prompt,li2024position,ren2024advances} or RSs~\cite{liu2023pre,wu2023survey}, to the best of our knowledge, no existing work has systematically analyzed or discussed the integration of FMs into FRSs. Our paper aims to fill this gap by providing a comprehensive examination of this intersection.

\textbf{Contributions.} % Write our contribution here
Our main contributions are as follows:
\begin{itemize}
    \item We establish a comprehensive framework for applying FMs to FRSs, elaborating on the underlying principles and methodologies for effective integration.

    \item By thoroughly analyzing existing technologies, we inspire innovation in leveraging the pre-training capabilities of FMs within FRSs, highlighting potential advancements.

    \item We delve into the challenges and practical issues of integrating FMs into FRSs, including privacy protection, data heterogeneity, communication efficiency, and model generalization, providing insights and potential solutions.

    \item We identify current research gaps and outline future directions, aiming to guide subsequent academic research and technological development in this emerging area.

    \item Through application studies, we illustrate how the integration of FMs with FRSs can be applied in real-world scenarios, bridging the gap between theory and practice.
\end{itemize}

By elucidating the integration of FMs and FRSs, our paper seeks to promote further exploration and innovation, facilitating rapid advancement and broader adoption in the field.



% This survey aims to provide a clear theoretical framework for applying FMs to FRSs and to elaborate on their principles and methods of application. 
% By analyzing existing technologies, this paper strives to drive innovation in integrating the pre-training capabilities of FMs into FRSs. 
% The article discusses in detail the technical challenges and practical issues faced when integrating FMs, such as privacy protection, data heterogeneity, communication efficiency, and model generalization capabilities. 
% It also identifies current research gaps and future directions, aiming to guide subsequent academic research and technological development. 
% Additionally, through application studies, this paper demonstrates how to apply the integration of FMs with FRSs in practical scenarios, thereby deepening the integration of theory and practice.


==> TKDE/sections/sec_res.tex <==
%!TEX root = ../main.tex

\section{Resources}
\label{sec:res}

In this section, we introduce the commonly used datasets and evaluation metrics in FRS. 
The aim is to provide a comprehensive overview of the resources used in the field, helping readers understand the types of materials and benchmarks typically employed. 
This section presents various datasets, including explicit and implicit feedback types, along with metrics for evaluating recommendation performance. 
These datasets and metrics are crucial for assessing and improving the effectiveness of FRSs.

\subsection{Datasets}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/type_feedback.png}
    \caption{Two types of Feedbacks.}
    \label{fig:type_feedback}
\end{figure}


\begin{table*}[!htbp]
\centering
\caption{Datasets with Explicit Feedback.}
\resizebox{.95\textwidth}{!}{
\begin{tabular}{clcccccccc}
\hline
                            & \multicolumn{1}{c}{}                          &                          &                          &                              &                            & \multicolumn{4}{c}{Context}                                                                                                                   \\
\multirow{-2}{*}{}          & \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multirow{-2}{*}{\#User} & \multirow{-2}{*}{\#Item} & \multirow{-2}{*}{\#Feedback} & \multirow{-2}{*}{Sparsity} & User                              & Item                              & Feedback                          & Timestamp                         \\ \hline
                            & Amazon Beauty                                 & 1,210,271                & 249,274                  & 2,023,070                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Books                                  & 8,026,324                & 2,330,066                & 22,507,155                   & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon CDs                                    & 1,578,597                & 486,360                  & 3,749,004                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Cell Phone                             & 2,261,045                & 319,678                  & 3,447,249                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Clothing                               & 3,117,268                & 1,136,004                & 5,748,920                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Games                                  & 826,767                  & 50,210                   & 1,324,753                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Garden                                 & 714,791                  & 105,984                  & 993,490                      & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Home                                   & 2,511,610                & 410,243                  & 4,253,926                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Kindle                                 & 1,406,890                & 430,530                  & 3,205,467                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Movies                                 & 2,088,620                & 200,941                  & 4,607,047                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Music                                  & 478,235                  & 266,414                  & 836,006                      & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Sports                                 & 1,990,521                & 478,898                  & 3,268,695                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Toys                                   & 1,342,911                & 327,698                  & 2,252,771                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-14}{*}{Amazon Reviews}   & Amazon Video                                  & 426,922                  & 23,965                   & 583,933                      & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & ML-100K                                       & 943                      & 1,682                    & 100,000                      & 93.70\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & ML-1M                                         & 6,040                    & 3,952                    & 10,000,209                   & 95.81\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & ML-10M                                        & 69,878                   & 10,681                   & 10,000,054                   & 98.69\%                    & {\color[HTML]{00B050} \textbf{}}  & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-4}{*}{MovieLens} & ML-20M                                        & 138,493                  & 27,278                   & 20,000,263                   & 99.47\%                    & {\color[HTML]{00B050} \textbf{}}  & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & Yelp2018                                      & 1,326,101                & 174,567                  & 5,261,669                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2020                                      & 1,968,703                & 209,393                  & 8,021,122                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2021                                      & 2,189,457                & 160,585                  & 8,635,403                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2022                                      & 1,987,929                & 150,346                  & 6,990,280                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-5}{*}{Yelp}      & Yelp-full                                     & 5,556,436                & 539,254                  & 28,908,240                   & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & Anime                                         & 73,515                   & 11,200                   & 7,813,737                    & 99.05\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   &                                   \\
                            & Book Crossing                                 & 105,284                  & 340,557                  & 1,149,780                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                            & Douban                                        & 738,701                  & 28                       & 2,125,056                    & 89.73\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Epinions                                      & 116,260                  & 41,269                   & 188,478                      & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Goodreads                                     & 876,145                  & 2,360,650                & 228,648,342                  & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Jester                                        & 73,421                   & 101                      & 4,136,360                    & 44.22\%                    &                                   &                                   &                                   &                                   \\
                            & Netflix                                       & 480,189                  & 17,770                   & 100,480,507                  & 98.82\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yahoo Music                                   & 1,948,882                & 98,211                   & 11,557,943                   & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\ \hline
\end{tabular}
}
\label{tab:explicit}
\end{table*}


\begin{table*}[!htbp]
\centering
\caption{Datasets with Implicit Feedback.}
\resizebox{.95\textwidth}{!}{
\begin{tabular}{clcccccccc}
\hline
                         & \multicolumn{1}{c}{}                          &                          &                          &                              &                            & \multicolumn{4}{c}{Context}                                                                                                                   \\
\multirow{-2}{*}{}       & \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multirow{-2}{*}{\#User} & \multirow{-2}{*}{\#Item} & \multirow{-2}{*}{\#Feedback} & \multirow{-2}{*}{Sparsity} & User                              & Item                              & Feedback                          & Timestamp                         \\ \hline
                         & MIND\_large\_train                            & 711,223                  & 27,047                   & 83,507,374                   & 99.57\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & MIND\_large\_dev                              & 255,991                  & 6,998                    & 14,085,557                   & 99.21\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & MIND\_small\_train                            & 50,001                   & 20,289                   & 5,843,444                    & 99.42\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-4}{*}{MIND}   & MIND\_small\_dev                              & 50,001                   & 5,370                    & 2,740,998                    & 98.98\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                         & QK-video                                      & 5,022,750                & 3,753,436                & 142,321,193                  & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                         & QK-article                                    & 1,325,838                & 220,122                  & 46,111,728                   & 99.98\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                         & QB-video                                      & 34,240                   & 130,647                  & 1,701,171                    & 99.96\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
\multirow{-4}{*}{Tenrec} & QB-article                                    & 24,516                   & 7,355                    & 348,736                      & 99.81\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\ \hline
                         & Adressa                                       & 15,514                   & 923                      & 2,717,915                    & 81.02\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Foursquare                                    & 1,083                    & 38,333                   & 227,428                      & 99.45\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Gowalla                                       & 196,591                  & 950,327                  & 6,442,890                    & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} \checkmark} & {\color[HTML]{00B050} \checkmark} \\
                         & Last.FM                                       & 1,892                    & 17,632                   & 92,834                       & 99.72\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Pinterest                                     & 55,187                   & 9,911                    & 1,445,622                    & 99.74\%                    &                                   &                                   &                                   &                                   \\
                         & Steam                                         & 2,567,538                & 32,135                   & 7,793,069                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                         & TaFeng                                        & 32,266                   & 23,812                   & 817,741                      & 99.89\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                         & Tmall                                         & 963,923                  & 2,353,207                & 44,528,127                   & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\ \hline
\end{tabular}
}
\label{tab:implicit}
\end{table*}

As shown in Fig. \ref{fig:type_feedback}, the datasets used can be categorized into two types based on user feedback in FRS: explicit feedback and implicit feedback.
Explicit feedback includes direct responses from users about their preferences. 
This typically includes ratings (such as a 1-5 scale), user comments, and like/dislike statements. 
Such data provides straightforward insights into user preferences, making it highly valuable for training recommendation models.
Common datasets with explicit feedback include the following shown in Table~\ref{tab:explicit}: 
\begin{itemize}
    \item Amazon Reviews\footnote{https://cseweb.ucsd.edu/~jmcauley/datasets.html\#amazon\_reviews}: The Amazon Reviews dataset is a large-scale dataset that contains product information across various categories such as Books, CDs, and Music. It includes reviews (ratings, text, helpfulness votes) and product metadata (description, category information, price, brand, and image features). There are three updated versions of this dataset from the years 2014~\cite{mcauley2015image,he2016ups}, 2018~\cite{ni2019justifying}, and 2023~\cite{hou2024bridging}.
    \item MovieLens Datasets\footnote{https://grouplens.org/datasets/movielens/}: The MovieLens datasets~\cite{harper2015movielens}, initially released in 1998, capture individuals' stated movie preferences. These preferences are recorded as tuples, with each tuple showing a person's rating (from 0 to 5 stars) for a movie at a specific time. Users enter these ratings through the MovieLens website, which provides personalized movie suggestions based on these ratings.
    \item Yelp Datasets\footnote{https://www.yelp.com/dataset}: This dataset is a subset of Yelp's business, review, and user data. It was initially developed for the Yelp Dataset Challenge, which allows students to study or analyze Yelp data and present their insights. In total, there are four versions of the Yelp datasets.
    \item Anime\footnote{https://www.kaggle.com/datasets/CooperUnion/anime-recommendations-database}: It collects user preference data from the MyAnimeList website, and contains information from 73,516 users on 12,294 anime titles. Users can add anime to their completed list and rate them, and this dataset compiles these ratings.
    \item Book Crossing\footnote{https://grouplens.org/datasets/book-crossing/}: The Book-Crossing dataset is a well-structured collection of data collected by Cai-Nicolas Ziegler in a 4-week crawl from the Book-Crossing community. This dataset primarily comprises user interactions that include book ratings, ranging from 0 to 10. 
    \item Douban\footnote{https://www.kaggle.com/datasets/utmhikari/doubanmovieshortcomments}: The Douban Movie dataset is a Chinese website where internet users can post their opinions and comments about films. It contains over 2 million short comments on 28 movies from the Douban Movie website.
    \item Epinions\footnote{https://cseweb.ucsd.edu/~jmcauley/datasets.html\#social\_data} \cite{cai2017spmc}: This dataset was collected from Epinions.com, a popular online consumer review site. It includes trust relationships between users and covers a period from January 2001 to November 2013.
    \item Goodreads\footnote{https://www.kaggle.com/datasets/jealousleopard/goodreadsbooks}: This dataset includes reviews from the book review website Goodreads, along with various attributes describing the books. Importantly, the dataset captures different levels of user interaction, from adding books to a shelf, to rating them, to reading them.
    \item Jester\footnote{https://eigentaste.berkeley.edu/dataset/}: It focuses exclusively on jokes. Users of the Jester online platform rate jokes and these ratings are then used to personalize joke recommendations for them.
    \item Netflix\footnote{https://www.kaggle.com/datasets/netflix-inc/netflix-prize-data}: Netflix provided a training dataset consisting of 100,480,507 ratings from 480,189 users for 17,770 films. The user and the movie are identified by integer IDs, and the rating scores range from 1 to 5 stars, also as integers.
    \item Yahoo Music\footnote{https://webscope.sandbox.yahoo.com/catalog.php?datatype=r}: It is known for its diversity and large scale. It contains a large collection of user ratings on different musical elements such as artists and genres.
\end{itemize}

Implicit feedback, on the other hand, is derived from user actions that indirectly indicate preferences, such as bookmarks, video/music play history, or click-throughs. Although implicit feedback does not directly express user likes or dislikes, it is rich and captures user behaviour more comprehensively.
\begin{itemize}
    \item MIND\footnote{https://msnews.github.io/}~\cite{wu2020mind}: The MIND dataset, sourced from the Microsoft News website, is a large-scale collection of approximately 160,000 English news articles and over 15 million user interaction records. It has been designed to advance research in news recommendation systems. It includes detailed textual content for each story and anonymized user interaction data to ensure privacy.
    \item Tenrec\footnote{https://github.com/yuangh-x/2022-NIPS-Tenrec}~\cite{yuan2022tenrec}: The Tenrec dataset is a comprehensive benchmark dataset for RSs, featuring user interactions from two recommendation platforms across four dataset files: QK-video and QB-video for video actions, and QK-article and QB-article for article actions.
    \item Adressa\footnote{https://reclab.idi.ntnu.no/dataset/}~\cite{gulla2017adressa}: It is a corpus of Norwegian news articles related to anonymous users. It is a collaborative project between the Norwegian University of Science and Technology and Adressavisen. The objective is to gain insight into the nature of news articles and their readers.
    \item Foursquare\footnote{https://sites.google.com/site/yangdingqi/home/foursquare-dataset}~\cite{yang2014modeling}: This dataset comprises check-in data from New York City, collected over a period of approximately ten months (from 12 April 2012 to 16 February 2013). It encompasses 227,428 check-ins in New York City, with each check-in recorded with its timestamp, GPS coordinates, and detailed venue category.
    \item Gowalla\footnote{https://snap.stanford.edu/data/loc-gowalla.html}~\cite{cho2011friendship}: Gowalla is a location-based social networking website where users can post their whereabouts by checking in. The dataset comprises data collected from the public API, which represents an undirected friendship network with 196,591 nodes and 950,327 connections. Additionally, it records 6,442,890 check-ins made by these users between February 2009 and October 2010.
    \item Last.FM\footnote{https://grouplens.org/datasets/hetrec-2011/}~\cite{Cantador:RecSys2011}: The Last.FM dataset represents a valuable resource that has been extensively utilized in the field of music information retrieval and RSs. It captures detailed information regarding music listening events from users. Each listening event is further enhanced with user demographics and specific descriptors that reflect their music tastes and consumption behaviours. 
    \item Pinterest\footnote{https://github.com/edervishaj/pinterest-recsys-dataset}~\cite{geng2015learning}: The Pinterest dataset represents a valuable resource for a variety of research and analytical purposes. It encompasses a diverse range of data, including images, user features, interests, and user interactions. 
    \item Steam\footnote{https://github.com/kang205/SASRec}~\cite{kang2018self}: Steam is a collection of information about games published on the Steam platform. It includes details such as game names, release dates, genres, developers, publishers, and other relevant information. 
    \item TaFeng\footnote{https://www.kaggle.com/datasets/chiranjivdas09/ta-feng-grocery-dataset}: TaFeng is a comprehensive collection of supermarket shopping data, including detailed transaction records from the Ta Feng supermarket in Taiwan, covering a period from November 2000 to February 2001. The dataset comprises a variety of data points, including customer demographics, product categories, and detailed item descriptions along with quantities purchased.
    \item Tmall\footnote{https://tianchi.aliyun.com/dataset/53}\cite{tmall18dataset}: The Tmall dataset is a comprehensive collection from Tmall, comprising anonymized user shopping records over a six-month period up to and including the "Double 11" event. It should be noted that the data is selectively sampled to address privacy concerns.
\end{itemize}

Both types of feedback play a critical role in the development of FRSs, providing diverse insights into user preferences that help improve the recommendation accuracy and relevance.


\begin{figure*}[!t]
    \centering
    \includegraphics[width=.95\textwidth]{figures/framework.pdf}
    \caption{
        A potential unified framework for FRSs integrates server-side global aggregation and hyperparameter optimization with client-side data processing, model training, and evaluation.
        }
    \label{fig:framework}
 \end{figure*}   


\subsection{Metrics}
\label{sec:metrics}

In the field of FRSs, the use of evaluation metrics is fundamental to assessing and refining the performance of our algorithms. Metrics serve as a quantitative lens through which we can observe how closely the system's suggestions match users' actual interests and preferences.

For predicting how well a system can estimate user preferences, there are several metrices measuring the prediction errors to judge the accuracy of the predictions \cite{shani2011evaluating}, such as Mean Absolute Error, Mean Squared Error and Root Mean Squared Error.
When it comes to classifying items, i.e., determining whether a user will like a product or not, we look at metrics such as Precision, Recall, Hit Ratio, F1 Score, Accuracy and AUC. 
These tell us how correctly the RS is classifying items, and the F1 score helps us balance the Precision and Recall.
%
Then to measure the item ranking ability, which is about listing recommendations in the right order, Average Precision and Mean Average Precision are key to this, as they assess the quality of the order of recommendations. 
Metrics such as Mean Reciprocal Rank \cite{voorhees2001trec}, Normalized Mutual Rank \cite{flanagan2021federated} and Normalised Discounted Cumulative Gain \cite{he2015trirank} also contribute by assessing how well the top recommended items are ranked.

On a broader scale, we consider recommendation-centric metrics such as Diversity, which ensures that a variety of items are suggested, and Coverage, which measures how many items from the catalogue are recommended. There are also some user-centric metrics include Novelty, which measures how new or surprising the recommendations are, and Degree of Agreement (DOA) \cite{wu2021hierarchical}, which quantifies the level of concordance between the ranking of items produced by a recommendation system and the ranking preferred by the user. 
Moreover, business metrics such as Click-Through Rate \cite{bian2023feynman} are critical to assessing the system's impact on user engagement and the company's bottom line, and Conversion Rate \cite{bian2023feynman} measures how efficient an algorithm is at providing recommendations that lead to user purchases.
There also are some metrics for measuring other functionality. 
For example, Gini Index \cite{castells2021novelty} evaluates the fairness of recommendation distribution, with lower values indicating more equitable distribution across items.



\subsection{Open-source framework}


Although there are already mature open-source frameworks for both RSs \cite{zhou2023mmrec,recbole[1.0],recbole[2.0],recbole[1.2.0]} and FL \cite{beutel2020flower,liu2021fate,openfl_citation}, there remains a significant gap when it comes to FRSs. 
Currently, there is no mature, unified, and widely applicable open-source framework specifically designed for FRSs.
%
Efforts such as FedMR\footnote{https://github.com/mtics/FedMR} \cite{li2024personalized} attempt to bridge this gap by integrating features from existing frameworks like MMRec\footnote{https://github.com/enoche/MMRec} \cite{zhou2023mmrec} and RecBole\footnote{https://github.com/RUCAIBox/RecBole} \cite{zhou2023mmrec}, extending them into the realm of federated multimodal recommendation. 
However, FedMR is still in its infancy and does not yet provide the robustness or general applicability required of a comprehensive solution for FRSs.

As illustrated in Fig. \ref{fig:framework}, we make a preliminary attempt to propose a potential unified framework for FRSs in this paper, which aims to ideally encompass the following:

\begin{itemize}
    \item \textbf{Integration of RSs and FL}: 
    Such a framework should seamlessly integrate the strengths of traditional recommendation systems with privacy-preserving capabilities from federated learning, addressing both data heterogeneity and privacy constraints effectively.
    
    \item \textbf{Modular and Extensible Architecture}: 
    The framework should feature a modular design that separates core components such as data preprocessing, model training, evaluation, and aggregation, facilitating improvements and the easy integration of new modules or functionalities.
    
    \item \textbf{Support for Multimodal Data}: 
    Leveraging the strengths of multimodal models, the framework should support the incorporation of various data modalities, enabling a more comprehensive understanding of user preferences and improving recommendation accuracy.
    
    \item \textbf{Scalability and Device Adaptability}: 
    The framework must be capable of scaling to accommodate a large number of clients and adapt to heterogeneous devices with varying computational capabilities, ensuring efficient performance on resource-constrained devices.
    
    \item \textbf{Privacy and Security}: 
    The framework should incorporate advanced privacy-preserving mechanisms, such as differential privacy and secure multi-party computation, to guarantee data confidentiality during both training and communication phases.
\end{itemize}

Despite the absence of a mature open-source FRS framework, the existing building blocks in RS and FL frameworks provide a strong foundation. 
By extending these capabilities and overcoming the unique challenges posed by FRSs, our proposed framework serves as a step towards a widely adopted, unified solution that fully supports FRSs.


% \begin{itemize}
%     \item Integration of Recommendation and Federated Learning: Such a framework should seamlessly integrate the strengths of traditional recommendation systems with privacy-preserving capabilities from federated learning, addressing both data heterogeneity and privacy constraints effectively.

%     \item \textbf{Modular and Extensible Architecture:} The framework should feature a modular design that separates core components such as data preprocessing, model training, evaluation, and aggregation. This separation would facilitate improvements and the easy integration of new modules or functionalities.

%     \item \textbf{Support for Multimodal Data:} Leveraging the strengths of multimodal models, the framework should support the incorporation of various data modalities (e.g., text, images, audio), enabling a more comprehensive understanding of user preferences and improving recommendation accuracy.

%     \item \textbf{Scalability and Device Adaptability:} The framework must be capable of scaling to accommodate a large number of clients and adapt to heterogeneous devices with varying computational capabilities. Techniques like model compression and lightweight fine-tuning should be employed to ensure efficient performance on resource-constrained devices.

%     \item \textbf{Privacy and Security:} The framework should incorporate advanced privacy-preserving mechanisms, such as differential privacy and secure multi-party computation, to guarantee data confidentiality during both training and communication phases.

% \end{itemize}

% Despite the absence of a mature open-source FRS framework, the existing building blocks in RS and FL frameworks provide a strong foundation. By extending these capabilities and overcoming the unique challenges posed by FRS, future work could lead to the development of a widely adopted, unified framework that fully supports federated recommendation scenarios.

==> TKDE/sections/sec_tax.tex <==
%!TEX root = ../main.tex


\section{Federated Recommendation Systems with Foundation Models}
\label{sec:frs_w_fm}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/frs_fm.pdf}
    \caption{
        Integration framework of FRSs with FMs, illustrating the key challenges in three stages: Client Model Update, Communication, and Global Aggregation.
        }
    \label{fig:frs_fm}
 \end{figure}   

As illustrated in Fig. \ref{fig:frs_fm}, a typical FRS comprises three key stages: client model update, communication, and global aggregation~\cite{alamgir2022federated}. 
The integration of FMs aligns with these stages. 
This section provides a comprehensive overview by summarizing representative works at each stage and examining additional dimensions of integrating FMs into FRS.

\subsection{Client Model Update}

In FRS, clients have the following characteristics \cite{yang2020federated,alamgir2022federated}:
\begin{itemize}
\item \textbf{Data Sparsity}: 
As mentioned earlier, a major advantage of FRS is privacy. 
The data required for model training in FRS, such as user information and interaction history, is privacy sensitive and therefore must remain on the user's device, creating data silos. 
This approach not only complies with data privacy regulations (such as GDPR), but also increases user trust. 
However, this means that each user has a relatively small amount of data compared to the entire dataset, and each user only accesses a portion of the item set, leading to data sparsity.

\item \textbf{Non-IID Data}: 
Each client independently trains the model on its local data. This allows the model to better adapt to each user's unique preferences and behaviors, improving personalization and accuracy of recommendations. The resulting data distribution often does not satisfy the independent and identically distributed (IID) assumption, leading to the problem of data heterogeneity.

\item \textbf{Device Limitations}:
In addition, user devices are typically consumer products such as mobile phones and personal computers, which are characterized by unstable communication and limited computational resources. 
This requires keeping the computational load of the models deployed on the client and the amount of information exchanged with the server as low as possible.
\end{itemize}

FMs are typically pre-trained on large, diverse datasets, providing them with rich knowledge and strong representational capabilities. 
This pre-training endows them with prior knowledge that can be quickly adapted to specific client data through fine-tuning \cite{bommasani2021opportunities}. 
Therefore, FMs learn general feature representations, offering adaptability to different data distributions. 
Applying FMs during the client update phase in FRS can significantly enhance the performance of local models. 
Specifically, the advantages are outlined as follows:
\begin{itemize}

    \item \textbf{Addressing Data Sparsity}: 
    FMs can apply the knowledge learned from large corpora to local data through transfer learning \cite{zeng2024federated}. 
    For instance, a pre-trained FM can be effectively fine-tuned on a small amount of local data at the client to adapt to specific user behaviors, thereby achieving good performance in downstream tasks such as providing more accurate recommendations \cite{wu2023survey,yuan2024fellas}. 
    Furthermore, by fine-tuning the base model locally, sensitive data does not need to leave the device, protecting user privacy \cite{rame2023model}. 
    Thus, even with limited data, clients can achieve better model performance, alleviating the challenges brought by data sparsity.

    \item \textbf{Handling Non-IID Data}: FMs' strong representational capabilities enable them to capture complex user preferences and behaviors. 
    For example, FMs possess powerful semantic understanding abilities, allowing them to better interpret user search queries \cite{lu2020twinbert,liu2021pre}, comments \cite{liu2023pre}, and other textual data \cite{geng2022recommendation}, thereby providing recommendations that align more closely with user needs. 
    Moreover, FMs can learn complex patterns from non-IID data \cite{han2021pre,li2024feddae,tang2024higpt}, enhancing the model's adaptability to different user preferences and ensuring that recommendation results stay consistent with the user's current interests and needs. 
    Applying FMs during the client update phase can achieve a higher level of personalized recommendation, effectively addressing data heterogeneity.

    \item \textbf{Adapting to Device Limitations}: 
    Although fine-tuning and updating FMs typically require significant computational resources, optimizing the model architecture and employing lightweight fine-tuning techniques can reduce the computational burden on devices \cite{han2024parameter}. 
    The knowledge transfer capability of FMs allows for efficient local fine-tuning under limited computational resources, thereby achieving good recommendation performance even in resource-constrained environments \cite{chen2024percept,han2024parameter}. 
    Additionally, model compression techniques can be used to reduce the model size, thereby lowering computational and storage requirements to suit the limitations of user devices \cite{zhu2023survey}.

\end{itemize}

These characteristics make FMs highly suitable for addressing the diverse data requirements of clients in FRS, thereby improving the generalization performance of local models. 
% However, when faced with data that significantly deviates from the training distribution, FMs may experience performance degradation, a challenge known as out-of-distribution generalization \cite{rame2023model}. 
% Additionally, if there are biases in the training dataset, FMs may learn and reinforce these biases, leading to unfair outcomes across different data distributions \cite{glocker2023risk,hou2024large,wu2024exploring}.


\subsection{Communication}
Communication between clients and the server is a critical phase in FRSs, involving the transmission of model update information from each client to the central server. 
Ensuring efficiency and security during this process is essential for maintaining system performance and protecting user privacy. 
However, this phase faces significant challenges, including the high communication costs associated with transmitting large volumes of data and the inherent security risks of handling sensitive information. 
Below, we firstly outline these challenges as follows:

\begin{itemize}
    \item \textbf{Communication Costs:} 
    The transmission of large-scale model parameters, gradients, or other statistical data can result in excessive communication overhead. 
    This is especially problematic in systems with many clients or high-dimensional models, where bandwidth and latency constraints become bottlenecks.
    
    \item \textbf{Transmission Security:} 
    Sensitive data encapsulated in model updates may be vulnerable to interception during transmission. 
    Such breaches could lead to privacy violations or exposure of user data, undermining the privacy-preserving goals of FRS. 
    Although encryption techniques can mitigate these risks, they often increase the computational and communication burden.
\end{itemize}

Addressing these challenges requires innovative approaches that enhance both efficiency and security. FMs, with their advanced representation and compression capabilities, offer promising solutions to overcome these limitations:

\begin{itemize}
    \item \textbf{Reducing Communication Costs:} 
    FMs can perform semantic compression \cite{li2021cross, liu2022multi}, extracting critical features while eliminating redundant information, thus significantly reducing the data transmitted between clients and the server. 
    Furthermore, optimized communication protocols tailored to FM representations \cite{shahid2021communication} can further improve data exchange efficiency.
    
    \item \textbf{Enhancing Transmission Security:} 
    Transmitting sensitive data in FRSs poses significant privacy risks. 
    FMs enhance transmission security by transforming raw model updates into abstract representations that retain essential information while removing sensitive details, reducing the risk of privacy leakage \cite{ren2024advances}. 
    Additionally, FMs enable semantic compression \cite{gilbert2023semantic}, which not only reduces communication overhead but also minimizes the risk of adversarial attacks. 
    When combined with techniques such as secure aggregation \cite{kadhe2020fastsecagg}, FMs provide an efficient and scalable solution that strengthens both the security and performance of data transmission in FRS.

\end{itemize}





% \subsection{Communication}

% In FRS, communication between clients and the server is a critical phase. 
% The primary task at this stage is to transmit model update information from each client to the central server while ensuring data security and communication efficiency during the transmission process.
% In traditional FRS frameworks, communication between clients and the server typically involves transmitting large amounts of update information, which may include model parameters, gradients, or other relevant statistical data. To ensure efficient and secure communication, common strategies include data compression \cite{cheng2017survey,yang2021h,li2022soteriafl}, encrypted transmission \cite{qu2021secure,buyukates2022lightverifl}, and secure aggregation \cite{bonawitz2016practical,kadhe2020fastsecagg,fereidooni2021safelearn}. However, with the increasing data scale and higher privacy protection requirements, these traditional methods face significant challenges \cite{ren2024advances}.

% FMs, especially LLMs, possess strong representation capabilities, enabling them to extract key features from model updates through efficient data representation \cite{yuan2023power,marone2024data} and semantic compression techniques \cite{li2021cross,liu2022multi}. By removing redundant information and unnecessary data, and retaining only essential information, FM can transform this into a more compact representation, significantly reducing the data transmission volume between clients and the server. Optimizing communication protocols \cite{shahid2021communication} and enhancing data compression and security during this process can markedly improve the overall performance of the system.

\subsection{Global Aggregation}

In FRS, the global aggregation phase of the server is responsible for combining model updates from all clients into a single global model. This phase is of critical importance in ensuring the overall performance and effectiveness of personalized recommendations. Server global aggregation is characterized by the following key features \cite{qi2023model}:

\begin{itemize}
\item \textbf{Diverse Client Updates}: 
The server must handle updates from a large number of clients, each containing different data and user behaviors. 
To ensure the overall quality of the model and the accuracy of recommendations, the server must effectively integrate this diverse data.

\item \textbf{Noisy Data}: 
The global aggregation process must be sufficiently robust to handle potentially noisy data and anomalous updates from clients, which can adversely affect the global model's performance.

\item \textbf{Scalability}: 
The scalability of the server's global aggregation is critical, especially when dealing with a large number of clients and massive amounts of data. The system must efficiently process and aggregate updates to maintain performance.
\end{itemize}

To address these challenges, several existing strategies have been developed. For example, in each iteration, given resource constraints and privacy concerns, the central server may only communicate with a subset of clients. Studies \cite{chai2020secure,li2023federated} indicate that clients should not participate in successive training rounds, as attackers could potentially infer information about the client from transmitted gradients or model parameters. 
The client selection strategy determines which clients will participate in the current training round based on factors such as computational power, network stability, data diversity, and data quality \cite{cho2020client}. 
For example, client selection can be done by random sampling or based on statistical characteristics of the data to ensure that the model learns from diverse data sources, thereby increasing its generalization ability. 
However, these existing strategies have limitations, such as suboptimal aggregation efficiency and challenges in fully exploiting the contextual information present in client updates.

FMs can play a significant role in enhancing the global aggregation process.
Traditional aggregation methods, such as naive weighted averaging proposed in FedAvg \cite{mcmahan2017communication}, may not fully exploit the contextual information present in the data. 
FMs, however, are capable of intelligently aggregating updates by understanding the semantics and contextual relationships of each participant's updates \cite{wang2023seggpt}.
\begin{itemize}

    \item \textbf{Context-Aware Aggregation}: 
    FMs utilize their powerful representation capabilities to analyze the structural and statistical characteristics of client updates, including update frequency, scale, and trends. This enables the server to more effectively assess the significance of each update without relying on potentially sensitive user-specific information, thereby aligning the aggregation process more closely with system-wide patterns and requirements \cite{yu2023federated}.
    By understanding the latent relationships between updates, FMs assign appropriate weights to individual contributions, improving the fidelity of the global model.
    
    \item \textbf{Dynamic Weighting}: 
    FMs enable dynamic adjustment of update weights based on their relevance to the global model \cite{han2024parameter}. 
    For instance, updates contributing to under-represented data distributions may receive higher weights, ensuring that the global model remains inclusive and robust to diverse data sources \cite{duan2020self}.
    
    \item \textbf{Knowledge-Based Aggregation}: 
    Leveraging the extensive knowledge base of FMs \cite{rawte2023survey}, knowledge-based aggregation strategies have the ability to capitalize on FMs' knowledge and reasoning capabilities to enhance the aggregation process. 
    For instance, if certain clients lack sufficient data, FMs can use pertinent information from their knowledge base to infer relationships and patterns, thereby supplementing and improving the aggregation process to have better performance \cite{chen2024large}.
    
    \item \textbf{Anomaly Detection and Handling}: 
    FMs also excel in anomaly detection \cite{elhafsi2023semantic,xu2024customizing}. 
    Client updates may be influenced by various factors, leading to noisy or abnormal data \cite{sun2024survey}. 
    If these abnormal updates are directly used in global aggregation, they may affect the overall model quality. 
    FMs can analyze client updates to identify and handle anomalies, ensuring the robustness of global aggregation. 
    For example, if a client's data update shows a notable divergence from the majority, it may be regarded as noise or an anomaly, and FMs can choose to disregard or assign a reduced weight to it, thereby maintaining the stability of the global model \cite{liu2023pre}.
    
\end{itemize}

Overall, FMs effectively tackle the key challenges in the global aggregation phase by integrating client updates with context-awareness, dynamically weighting to handle noisy data, leveraging pre-trained knowledge for scalability, and performing robust anomaly detection. 
These approaches significantly enhance the global model's quality, robustness, and adaptability, positioning FMs as a promising tool for advancing FRSs. 
Continued research in this area could further unlock their potential, fostering progress in personalized, scalable, and privacy-preserving recommendations.



% Context-aware aggregation represents a critical application of FM in global server aggregation. Traditional aggregation methods, such as naive weighted averaging proposed in FedAvg \cite{mcmahan2017communication}, may not fully exploit the contextual information present in the data. 
% FM, however, is capable of intelligently aggregating updates by understanding the semantics and contextual relationships of each participant's updates \cite{wang2023seggpt}. To illustrate, when FM receives customer updates, it analyzes the contextual information of each update, such as user behavior patterns, preferences, and history. This information enables FM to better comprehend the significance and value of each update and to assign distinct weights accordingly \cite{yu2023federated}. 
% This context-aware aggregation method can more accurately reflect user preferences and behaviors, thereby enhancing the overall performance of the model. 
% Dynamic weighting permits the system to adapt more effectively to users' personal needs and to provide recommendations that are more aligned with their interests.

% With its extensive knowledge base \cite{rawte2023survey}, FM can utilize this knowledge to make more informed decisions during the aggregation process. Knowledge-based aggregation strategies can capitalize on FM's knowledge and reasoning capabilities to enhance the efficacy of aggregation. To illustrate, in the event that certain customers lack sufficient data, FM can leverage pertinent information from its knowledge base to infer relationships and patterns between data, thereby supplementing and improving aggregation.
% The key concept of Mixture of Experts (MoE) \cite{jacobs1991adaptive} is that different expert models specialize in different parts of a problem. By appropriately weighting and combining their outputs, better overall performance can be achieved. The MoE architecture has a similar function to aggregation strategies in FRS. Therefore, applying this architecture to the aggregation strategy in FRS may result in improved recommendation performance.

% In terms of anomaly detection, FM also performs exceptionally well \cite{elhafsi2023semantic,xu2024customizing}. In FRS, client updates may be influenced by various factors, leading to noisy or abnormal data \cite{sun2024survey}. If these abnormal updates are directly used in global aggregation, they may affect the overall quality of the model. FM can utilize its strong anomaly detection capabilities to analyze client updates, identify and handle these anomalies, ensuring the robustness of global aggregation. For instance, if a client's data update exhibits a notable divergence from the majority of client updates, it may be regarded as noise or an anomaly. FM has the capacity to elect to disregard or assign a diminished weight to it, thus reducing its deleterious impact on the global model and ensuring the stability and robustness of the global model. Liu et al. \cite{liu2023pre} observed in their study that FM is capable of effectively filtering out noisy data by identifying aberrant patterns, thereby enhancing the stability and reliability of the aggregation process.

% This application direction has considerable potential for future development and is worthy of further research and investigation.


==> sections/sec_app.tex <==
%!TEX root = ../main.tex

\section{Applications}
\label{sec:app}

\subsection{eHealthcare Systems}
 eHealthcare systems leverage modern technology to enhance the quality and efficiency of medical services, such as remote diagnosis and patient monitoring. Federated recommendation systems allow different medical institutions to share insights from patient data without sharing the data itself, which is crucial for protecting sensitive health information. Generative models use this data to provide doctors and patients with personalized treatment plans and health advice, improving diagnostic accuracy and treatment outcomes. Thus, federated recommendation systems combined with generative models can integrate patient health data across institutions to create complex treatment pathways and simulate disease progression, enabling doctors to better predict patients' responses to specific treatments and provide more precise medical services.

\subsection{Industrial Applications}
In manufacturing, automation and intelligent technologies significantly enhance production efficiency and safety. Federated recommendation systems foster technological collaboration between different enterprises by sharing non-sensitive data, accelerating product design and optimization processes. This not only shortens product development cycles but also protects corporate trade secrets. Generative models can design new mechanical parts or product prototypes by simulating different design variables, quickly proposing multiple design solutions; they can also help predict machine failures, perform maintenance in advance, and reduce downtime, thereby enhancing production efficiency. Federated recommendation systems combined with generative models enable the sharing of improvements and innovations while maintaining data privacy between companies.

\subsection{Consumer Services}
Analyzing consumer behavior helps businesses deeply understand customer needs. Federated recommendation systems can integrate data from different service providers while protecting user privacy, achieving personalized services. Generative models provide personalized recommendations based on this data, enhancing user experience. For example, in travel recommendation systems, models generate customized travel itineraries based on users' historical preferences. By simulating different consumer behavior patterns, businesses can predict market trends, adjust service strategies, and enhance competitiveness. Federated recommendation systems combined with generative models analyze user behavior data from different service providers to generate service plans that meet individual needs, promoting personalized service development.

\subsection{Retail and E-commerce}
Applying recommendation systems to online shopping and retail provides a personalized shopping experience. Federated recommendation systems in the retail and e-commerce sectors analyze consumer shopping habits to generate personalized product recommendations, increasing users' purchasing desire and satisfaction. Retailers and e-commerce platforms can use generative models to predict consumer buying behavior, thereby offering more accurate product recommendations, optimizing inventory, and enhancing sales efficiency. Federated recommendation systems combined with generative models allow retailers and e-commerce platforms to consider market conditions comprehensively, predicting consumer buying behavior and providing more precise product recommendations, optimizing inventory, and enhancing sales efficiency.

\subsection{Finance and Banking}
In the financial sector, recommendation systems use data analysis and prediction models to optimize financial services, applicable for credit assessments, stock market analysis, etc., offering clients tailored financial products. Federated recommendation systems ensure transaction data privacy while offering clients tailored financial products. Generative models can simulate market behaviors, predicting stock prices or financial product returns. These models help financial institutions formulate more accurate investment strategies while reducing risks. In finance, federated recommendation systems combined with generative models help financial institutions protect client privacy while simulating market changes and user behavior, offering advice on investment products and credit strategies, thereby enhancing clients' investment returns and satisfaction.

\subsection{Smart Cities}
In smart city applications, systems need to process and analyze large-scale urban data. From optimizing traffic flow to devising public safety strategies, federated recommendation systems can help city planners use resident data without directly sharing it to recommend strategies for improving public services and infrastructure, enhancing urban management efficiency and improving residents' quality of life. Additionally, using generative models to simulate the effects of different strategies can find optimal solutions for managing and allocating urban resources. For example, by simulating traffic flow, models can predict congestion and propose solutions, improving urban traffic efficiency. Federated recommendation systems combined with generative models can help city planners optimize resource allocation and management efficiency without sharing resident data.

\subsection{Social Networking}
 Social platforms facilitate interpersonal communication and information sharing online, using recommendation systems to suggest content to users, such as friends or topics of interest, to increase user engagement. Federated recommendation systems can enhance user engagement and satisfaction while protecting user privacy. Generative models can generate personalized content recommendations, enhancing user engagement and satisfaction while ensuring the protection of user privacy, increasing platform attractiveness and user retention.

\subsection{Education}
 In the field of education, using recommendation systems can improve teaching methods by making appropriate recommendations based on students' progress and abilities, providing a personalized learning experience. Generative models can generate personalized learning materials and courses based on students' progress and interests. These customized learning resources can enhance students' learning efficiency and interest. Federated recommendation systems combined with generative models can generate personalized learning paths based on students' feedback and learning history. By simulating teaching scenarios and student learning processes, these systems can provide resources that better meet individual learning needs.



==> sections/sec_bg.tex <==
%!TEX root = ../main.tex

\section{Background and Preliminary}
\label{sec:bg}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/typical_FRS.pdf}
    \caption{
        A framework for FRS, illustrating client-side local training with private data, server-side global aggregation, and update communication. 
        Local models integrate user and item embeddings with prediction networks, while the server aggregates local updates to enhance the global model, ensuring both privacy and personalization.
    }
    \label{fig:typical_FRS}
\end{figure}


To provide a concise yet profound overview of the current landscape in FRSs and FMs, we summarize the core principles and development trends in each field to lay the groundwork, which would be helpful for understanding how their integration can overcome the key challenges in FRS.

\subsection{Federated Recommendation Systems}

FRSs leverage federated learning to deliver personalized recommendations while preserving user privacy by ensuring that sensitive data remains on local devices. 
A typical FRS framework, as illustrated in Figure~\ref{fig:typical_FRS}, involves three key stages \cite{sun2024survey}: local model updates, secure transmission of these updates, and global aggregation at a central server. 
Although FRSs inherently protect users' data privacy, they still suffer from challenges such as limited and non-IID data at each client, which result in data sparsity and heterogeneity~\cite{yang2020federated}.

\paragraph{Data Distribution Paradigms in FRS.} 
The distribution of data across clients significantly affects model performance. 
In a \textbf{Horizontal FRS}, clients share a common feature space but maintain distinct data samples. This is typical when users interact with a shared set of items while generating personalized data, and the aggregation of their updates helps build a robust model \cite{zhang2023dual,li2024federated,zhang2024federated}. 
In a \textbf{Vertical FRS}, clients possess overlapping user sets with different feature spaces, allowing the secure integration of heterogeneous data, such as combining financial records with behavioral data, to enrich user profiles \cite{zhang2021vertical,cao2023privacy,mai2023vertical,wan2023fedpdd}. 
When individual data sources are extremely limited, a \textbf{Transfer FRS} \cite{zhuang2020comprehensive,zhang2024transfr} employs transfer learning to share knowledge across domains, thereby mitigating data scarcity.

\paragraph{Communication Architectures in FRS.} 
The architecture that governs client-server communication is critical for ensuring efficiency and security in real-world applications. 
In a \textbf{Centralized FRS}, a central server collects and aggregates client updates, which simplifies the aggregation process but may introduce a single point of failure and potential privacy risks~\cite{li2022federated,zhang2023lightfr,zhang2023dual,li2024federated,zhang2024federated,zhang2024transfr}. Alternatively, a \textbf{Semi-decentralized FRS} uses intermediate nodes such as edge servers to reduce communication overhead while balancing efficiency and privacy~\cite{qu2023semi}. In a \textbf{Decentralized FRS}, peer-to-peer communication eliminates the need for central coordination, thereby enhancing privacy though at the cost of increased network complexity~\cite{hegedHus2019decentralized,zheng2023decentralized,li2024decentralized}.

\subsection{Foundation Models}

Recent breakthroughs in hardware, transformer architectures, and large-scale datasets have given rise to Foundation Models, which are capable of transferring learned knowledge across a wide array of tasks~\cite{bommasani2021opportunities,kaplan2020scaling,isik2024scaling}. By definition, a foundation model is trained on extensive data via self-supervised learning and can be adapted to diverse downstream applications through techniques such as fine-tuning or prompting~\cite{bommasani2021opportunities}. Models like GPT-3 exemplify these systems, showcasing properties of \textit{emergence}—the spontaneous development of novel capabilities—and \textit{homogenization}—a unified approach to varied tasks.

\paragraph{Training Data Types in FMs.} The capabilities of FMs are largely determined by the nature of their training data. \textbf{Language FMs} are trained on vast textual corpora and excel in natural language understanding, translation, and text generation~\cite{devlin2018bert,liu2019roberta,brown2020language,touvron2023llama}. \textbf{Vision FMs}, developed using large-scale image datasets, are tailored for visual tasks such as object recognition and segmentation, capturing complex visual patterns~\cite{dosovitskiy2020image,wang2023all,zhang2023recognize,kirillov2023segment}. \textbf{Multi-modal FMs} integrate different data modalities, such as text and images, to support cross-modal applications and deliver richer representations~\cite{radford2021learning,tamkin2021understanding}.

\paragraph{Functional Objectives in FMs.} FMs are also categorized by their functional objectives. \textbf{Discriminative FMs} are designed to make fine-grained distinctions between inputs, making them ideal for classification and regression tasks~\cite{yao2022prompt,chen2023robust,ali2023evaluating}. In contrast, \textbf{Generative FMs} learn the underlying data distribution to synthesize new data instances, a capability demonstrated by models such as GPT-3 and DALL·E~\cite{cao2023comprehensive,otter2020survey,ho2022cascaded,saharia2022palette}.

\paragraph{Adaptation Techniques for FMs.} To customize FMs for specific tasks without retraining the entire model, various adaptation techniques have been developed. \textbf{Prompt-based fine-tuning} employs learnable prompts to guide model behavior with minimal modifications~\cite{zhou2022learning,zhou2022conditional}. \textbf{Adapter-based fine-tuning} involves inserting small, trainable modules into the pre-trained network, thereby confining updates to these components while preserving the majority of the original parameters~\cite{guo2023calip,gao2024clip,hu2021lora}. \textbf{External knowledge-based adaptation} further enhances performance by incorporating supplementary information, such as domain-specific data or knowledge graphs, into the model’s learning process~\cite{pratt2023does,yang2023language}.

\subsection{Motivation for Integrating FMs into FRSs}

Despite their robust privacy preservation, FRSs are hampered by data sparsity and heterogeneity due to the isolation of client data. In contrast, FMs are endowed with rich, transferable knowledge from large-scale pre-training, enabling them to capture complex patterns and semantic nuances across diverse datasets. Integrating FMs into FRSs offers a promising solution: by leveraging the generalized representations of FMs, local models can be enhanced and global aggregation can be more effectively guided. This synergy not only addresses the limitations of isolated data but also paves the way for more accurate, scalable, and privacy-aware recommendation systems.

In summary, while FRSs and FMs have each made significant strides independently, their integration holds the promise of overcoming longstanding challenges in personalized recommendation. This background sets the stage for the subsequent exploration of the future prospects and challenges associated with uniting these two transformative paradigms.










% \section{Background and Preliminary}
% \label{sec:bg}

% To provide a comprehensive understanding of the integration of FRSs and FMs, this section outlines their core principles, taxonomies, and foundational structures. 
% This background establishes the basis for analyzing the synergies between these two paradigms.
% Moreover, The classification standards and adaptation techniques provide a structured framework for understanding the design and customization of both FRSs and FMs, highlighting the distinct challenges and opportunities.


% \subsection{Federated Recommendation System}

% \begin{figure}[!htbp]
%     \centering
%     \includegraphics[width=1.\columnwidth]{figures/typical_FRS.pdf}
%     \caption{
%         A framework for FRS, illustrating client-side local training with private data, server-side global aggregation, and update communication. 
%         Local models integrate user and item embeddings with prediction networks, while the server aggregates local updates to enhance the global model, ensuring both privacy and personalization.
%     }
%     \label{fig:typical_FRS}
% \end{figure}

% \begin{definition}[Federated Recommendation System]
% \label{def:frs}
% Federated Recommendation Systems employ federated algorithms for personalized information filtering, enhancing recommendation accuracy and service effectiveness while preserving user privacy by ensuring that users' sensitive data remains on their local devices. \looseness=-1
% \end{definition}

% FRSs enable collaborative learning across multiple clients without the direct exchange of raw user data. As depicted in Fig.~\ref{fig:typical_FRS}, an FRS typically involves three key processes: (1) local model updates on the client side, (2) communication of these updates, and (3) global aggregation at a central server. Moreover, FRSs can be categorized based on both data distribution and communication architecture~\cite{yang2020federated,sun2024survey}.

% \subsubsection{Data Distribution Paradigms in FRS}
% The way data is distributed across clients in FRSs directly affects collaboration and model performance. Three primary paradigms emerge in this context:

% \noindent \textbf{Horizontal FRS}: In horizontal FRS, clients share a similar feature space but possess distinct samples. This setup is common when users interact with a common set of items yet generate personalized data. Model updates from these clients are aggregated to build a robust recommendation model while preserving privacy~\cite{zhang2023dual,li2024federated,zhang2024federated}.  

% \noindent \textbf{Vertical FRS}: Vertical FRS applies when clients have overlapping sample sets but differ in feature spaces. This paradigm enables the secure integration of heterogeneous data, such as combining a bank's credit history with other user information, to enrich user profiles~\cite{zhang2021vertical,cao2023privacy,mai2023vertical,wan2023fedpdd}.  

% \noindent \textbf{Transfer FRS}: In scenarios where individual data sources are limited, Transfer FRS leverages transfer learning to share knowledge across domains. This approach proves especially valuable when standalone models suffer from data scarcity, allowing the system to benefit from related domains~\cite{zhuang2020comprehensive,zhang2024transfr}. \looseness=-1

% \subsubsection{Communication Architectures in FRS}
% The architecture governing client-server communication plays a critical role in FRS design, influencing both efficiency and privacy. Three typical architectures are recognized: 

% \noindent \textbf{Centralized FRS}: In centralized architectures, a central server collects and aggregates client updates. This method simplifies model aggregation but creates a single point of failure and may expose privacy risks due to reliance on a central entity~\cite{li2022federated,zhang2023lightfr,zhang2023dual,li2024federated,zhang2024federated,zhang2024transfr}.  

% \noindent \textbf{Semi-decentralized FRS}: Semi-decentralized architectures introduce an intermediate layer (e.g., edge servers) to reduce communication overhead. This design strikes a balance between the efficiency of centralized systems and the enhanced privacy offered by distributed architectures~\cite{qu2023semi}.  

% \noindent \textbf{Decentralized FRS} In decentralized FRS, peer-to-peer communication eliminates the need for central coordination. While this approach maximizes privacy by distributing control among clients, it also increases the complexity of network coordination~\cite{hegedHus2019decentralized,zheng2023decentralized,li2024decentralized}.


% \subsection{Foundation Model}

% Recent advances in hardware, transformer architectures, and large-scale datasets have driven the emergence of Foundation Models (FMs)~\cite{bommasani2021opportunities}. According to Stanford HAI~\cite{bommasani2021opportunities}, a foundation model is defined as follows:

% \begin{definition}[Foundation Model]
% \label{def:fm}
% A foundation model is any model trained on extensive data (typically via large-scale self-supervised learning) that can be adapted to a wide range of downstream tasks through fine-tuning or prompting.
% \end{definition}

% FMs such as GPT-3~\cite{brown2020language} exhibit two key properties~\cite{bommasani2021opportunities}: \textit{Emergence} (the spontaneous development of novel capabilities from training data) and \textit{Homogenization} (a unified approach that applies across diverse tasks). Despite their success, the limitations and failure modes of FMs remain underexplored~\cite{bommasani2021opportunities,wei2022chain,yang2024foundation,zhao2024explainability}. Moreover, OpenAI's Scaling Law~\cite{kaplan2020scaling,isik2024scaling} suggests that model performance scales as a power-law function of computational resources, parameters, and data size. Similar to FRSs, FMs can be classified based on the type of training data and their functional objectives.

% \subsubsection{Training Data Types in FM}
% The type of training data fundamentally shapes the capabilities of FMs, and are primarily divided into three categories based on the data they used during training:

% \noindent \textbf{Language FM}: These models are trained on extensive textual data and are tailored for natural language processing tasks. Their broad exposure to diverse text corpora enables them to perform well in language understanding, translation, and text generation tasks~\cite{devlin2018bert,liu2019roberta,brown2020language,touvron2023llama}.  

% \noindent \textbf{Vision FM}: Vision FMs are developed using large-scale image datasets and are designed for tasks such as object recognition and segmentation. Their specialized training on visual data allows them to capture complex visual patterns essential for image analysis~\cite{dosovitskiy2020image,wang2023all,zhang2023recognize,kirillov2023segment}.  

% \noindent \textbf{Multi-modal FM}: By integrating multiple data modalities (e.g., text and images), multi-modal FMs support cross-modal applications. This fusion of diverse data types enables the model to handle tasks that require understanding and correlating information from different sources~\cite{radford2021learning,tamkin2021understanding}.

% \subsubsection{Functional Objectives in FM}
% Beyond training data, FMs are also categorized by their primary functional objectives, which determine how they process and generate information:

% \noindent \textbf{Discriminative FM}: Discriminative models are designed to differentiate between various input classes and are primarily used for classification and regression tasks. Their strength lies in their ability to make fine-grained distinctions among inputs~\cite{yao2022prompt,chen2023robust,ali2023evaluating}.  

% \noindent \textbf{Generative FM}: In contrast, generative models learn the underlying data distribution to create new data instances. Models such as GPT-3 and DALL·E exemplify this category, demonstrating remarkable capabilities in synthesizing text and images~\cite{cao2023comprehensive,otter2020survey,ho2022cascaded,saharia2022palette}.

% \subsubsection{Adaptation Techniques}
% To tailor FMs for specific downstream tasks without retraining the entire network, various adaptation techniques have been developed. These methods allow for efficient fine-tuning by updating only a fraction of the model's parameters.  

% \noindent \textbf{Prompt-based Fine-tuning}: By leveraging learnable prompts that guide the FM’s behavior, it enables rapid adaptation to new tasks with minimal modifications~\cite{zhou2022learning,zhou2022conditional}. \looseness=-1

% \noindent \textbf{Adapter-based Fine-tuning}: By inserting small, trainable adapters into the pre-trained model, this technique confines updates to these modules, thereby preserving most of the original parameters while achieving task-specific customization~\cite{guo2023calip,gao2024clip,hu2021lora}. \looseness=-1

% \noindent \textbf{External Knowledge-based Adaptation}: This method incorporates additional external information, such as domain-specific data or knowledge graphs, to enhance the model's performance in specialized applications~\cite{pratt2023does,yang2023language}.


==> sections/sec_bio.tex <==
%!TEX root = ../main.tex

% \begin{IEEEbiographynophoto}{Zhiwei Li}
% Biography text here without a photo.
% \end{IEEEbiographynophoto}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/zhwl.jpg}}]{Zhiwei Li}
is pursuing his PhD at University of Technology Sydney. 
His research focuses on advancing personalized federated collaborative filtering by developing models that improve recommendation accuracy while ensuring user privacy. 
He has authored several influential papers, contributing to key areas of federated recommendation, including personalized item representations, multimodal data integration, and the application of foundation models in federated settings. 
He also serves as a reviewer for leading conferences, demonstrating his expertise.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/gdl1.jpg}}]{Guodong Long}
is a leading scholar in AI, and serves as Co-Director of the Representation Learning for Machine Intelligence Lab at University of Technology Sydney. 
His research focuses on trustworthy AI, personalized intelligence in federated learning, and on-device intelligence integrated with foundation models.
He has published about 150 papers, with over 24,000 citations (h-index: 50), featuring in top conferences like NeurIPS, ICML, and ICLR. 
In 2024, he ranked 21st globally in the AAAI/IJCAI domain on the AI 2000 Most Influential Scholars list.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/chxzh.jpg}}]{Chunxu Zhang}
completed her Doctoral degree at Jilin University, working on federated learning and recommender systems. 
She has published over 20 papers in top-tier venues (e.g., WWW, KDD, SIGIR, IJCAI, AAAI, and NeurIPS). 
In addition, she has been invited to be a reviewer for numerous distinguished conferences and journals such as WWW, KDD, ICLR, IJCAI, TNNLS, and TIFS.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/hlzh.jpg}}]{Honglei Zhang}
is currently pursuing his Ph.D. at Beijing Jiaotong University. 
During this period, he was a visiting scholar at Nanyang Technological University. 
His research work has been published on top-tier international venues, including ICDE, TOIS, and TNNLS. Additionally, he has been an PC and/or reviewer for many leading venues, such as WWW, NeurIPS, ICLR, TKDE and TOIS. 
His research interest primarily focuses on developing efficient and privacy-preserving recommender systems, with a particular interest in federated recommendation.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/jj1.jpg}}]{Jing Jiang}
is an ARC DECRA Fellow and an Associate Professor in the School of Computer Science and a core member of the Australian Artificial Intelligence Institute at University of Technology Sydney. 
Her research focuses on machine learning and its applications, with over 80 publications in top AI conferences and journals such as NeurIPS, ICML, ICLR, and IEEE TPAMI. 
Prof. Jiang has served as a program committee member for leading AI conferences and a reviewer for prestigious journals.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/bio/chqzh.jpg}}]{Chengqi Zhang}
is a leading expert in Distributed Artificial Intelligence and Data Mining, with over 388 publications and 34,500+ citations (H-index: 71)
As the founding Director of UTS’s Quantum Computation and Intelligent Systems Centre, he secured AU\$16.9 million in funding, establishing it as Australia’s top IT research hub and elevating UTS computer science into the global top 100 rankings.
His global influence is reflected in keynote talks at 33 major conferences and leadership roles, and His contributions have earned prestigious awards.
\end{IEEEbiography}


==> sections/sec_challenges.tex <==
%!TEX root = ../main.tex

\section{Key Challenges and Strategic Solutions}
\label{sec:challenge}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/challenges.pdf}
    \caption{
        Challenges in integrating FMs into FRSs, divided into data and model challenges, highlighting areas requiring strategic solutions for enhanced personalization and privacy.
        }
    \label{fig:chal}
 \end{figure}   

Integrating FMs into FRSs has introduced new opportunities for enhancing personalized recommendations while maintaining user privacy. 
However, as illustrated in Fig. \ref{fig:chal}, this integration presents significant challenges across multiple dimensions. 
Understanding these challenges comprehensively and developing effective strategies to address them is crucial for advancing FRSs. 
This section explores these challenges in depth and presents potential strategies to overcome them.


\subsection{Data Challenges and Mitigation Strategies}

\subsubsection{Privacy Concerns}
Privacy aims to prevent unauthorized access or misuse of data, especially during model training and data handling, to protect user identities and personal details \cite{hasan2023security}. 
In a federated setting, safeguarding user privacy is of utmost importance. 
Privacy concerns focus on preventing unintended exposure or misuse of personal data, ensuring that sensitive information remains confidential. 
While training and recommendations must occur without revealing personal data, FMs, such as GPT-3, may memorize and reproduce training data, potentially leaking sensitive information \cite{chen2023hide}. 
Additionally, if generated data closely resembles original data, user privacy risks may arise \cite{hasan2023security}.

To mitigate these privacy concerns, differential privacy \cite{minto2021stronger} can be employed by adding noise during model training to reduce data leakage risks while preserving model performance. 
Homomorphic encryption \cite{acar2018survey} allows training on encrypted data, effectively preventing data theft during transmission and processing. 
Moreover, machine unlearning techniques \cite{bourtoule2021machine} can be utilized to remove specific user data from the FMs, ensuring compliance with privacy regulations like GDPR.
An emerging approach, known as privacy rewrite, transforms sensitive data into anonymized formats before transmission. Frameworks like HaS \cite{chen2023hide} exemplify this by anonymizing private entities locally and reconstructing them after processing. This method reduces privacy risks, preserves data utility, and minimizes computational overhead. 

\subsubsection{Security Threats}
Security threats involve protecting data from malicious attacks or breaches \cite{hasan2023security}. 
While privacy controls who can access and use data, security emphasizes maintaining data integrity and defending against threats such as cyberattacks \cite{nasr2019comprehensive}. 
The integration of FMs into FRSs also necessitates ensuring data security, as participants may be subject to attacks like Member Inference Attacks \cite{nasr2019comprehensive}, Data Reconstruction Attacks \cite{lyu2021novel}, and Poisoning Attacks \cite{tolpegin2020data}, which can compromise model integrity or data quality.

To ensure data integrity and confidentiality during transmission, secure multi-party computation \cite{byrd2020differentially} can distribute computational tasks among multiple participants, preventing any single party from accessing complete data. Additionally, blockchain \cite{hai2022bvflemr,guo2023decentralized} can record data access and operations, enhancing data integrity, traceability, and transparency.

\subsubsection{Data Scarcity}
Despite FMs' potential to alleviate data sparsity, FRSs often face data scarcity, especially in scenarios where participants have limited interaction data under federated Settings \cite{alamgir2022federated}. 
Data sparsity can significantly impact model performance, particularly when user interactions are insufficient to build effective models.

Data augmentation techniques \cite{van2001art,mumuni2022data} can be used to generate diverse training samples, expanding the dataset size. Knowledge transfer \cite{chen2024percept} from rich datasets in other domains can also alleviate data sparsity, improving overall model performance. When employing generative FMs \cite{waqas2023revolutionizing,rossi2024augmenting}, quality control mechanisms are essential to ensure that synthetic data meets quality standards without introducing biases.

\subsubsection{Data Imbalance}
In federated settings, significant differences in data size and distribution exist across clients, causing data imbalance \cite{duan2020self,wang2021addressing,luo2022towards}. 
This imbalance, often driven by long-tail distributions of item labels and user behaviors, affects model training effectiveness.

To address sample imbalance, resampling techniques like oversampling minority classes or undersampling majority classes \cite{he2009learning} can be used. 
Weighted loss functions \cite{li2021autobalance,duan2020self} can also be used to assign higher importance to minority class samples during training, improving the capability to recognize underrepresented data without altering the data distribution.

\subsection{Model Challenges and Strategic Solutions}

\subsubsection{Synchronization Overhead}
In federated settings, the need for frequent synchronization between participants and the central server can result in high communication costs and system complexity, especially when dealing with large FMs with extensive parameters \cite{bommasani2021opportunities}.

Gradient compression \cite{lin2017deep} can help reduce the data transmitted during synchronization, thereby lowering communication costs. 
Asynchronous update strategies \cite{chen2019communication} that allow participants to update models independently, followed by periodic global synchronization, also enhance system efficiency.

\subsubsection{Client Heterogeneity}
Arising from variations in model types, sizes, and architectures, this issue creates challenges when deploying a unified FM in federated settings \cite{zhu2018knowledge}.

Adaptive training algorithms \cite{tian2019contrastive,zhang2021parameterized} that adjust model parameters based on each client's computational capabilities and data characteristics can address this issue. Knowledge transfer \cite{zhang2024transfr} between clients can further enhance model performance by mitigating disparities.

\subsubsection{Interpretability and Transparency}
FMs are often perceived as black-box models, which makes it challenging to understand their internal workings and may lead to issues with trust and compliance \cite{ren2024advances}.

Explainable AI \cite{gunning2019xai}, such as attention mechanisms \cite{mohankumar2020towards} and feature importance analysis \cite{carletti2019explainable}, offer insights into model decisions, enhancing transparency. 
Additionally, generative FMs \cite{schneider2024explainable} generate natural language explanations for recommendations, fostering user trust and acceptance.


















==> sections/sec_conclusion.tex <==
%!TEX root = ../main.tex

\section{Conclusion}
\label{sec:conclusion}

This paper has explored the integration of Federated Recommendation Systems with Foundation Models, demonstrating that leveraging pre-trained knowledge through lightweight adaptation effectively addresses challenges such as data sparsity, non-IID distributions, and device limitations while preserving user privacy. 
By enhancing both local model performance and global aggregation, this synergy mitigates key issues like privacy-performance trade-offs and communication bottlenecks. 
Looking forward, promising research avenues include generative data augmentation, cold-start mitigation, multi-modal fusion, and real-time adaptation, all of which are pivotal for developing robust, scalable, and user-centric recommendation systems. 
In essence, the fusion of FRSs and FMs offers a transformative pathway toward next-generation recommendation systems that are both highly effective and intrinsically privacy-preserving.


% This paper comprehensively examines the integration of FRSs with FMs, a direction that has gained attention for its ability to protect user privacy. 
% It begins by summarizing common approaches of FRSs and FMs, then delves into the challenges faced during integration. 
% To address these challenges, we comprehensively various strategies to adapt to data diversity, employing privacy-preserving methods, and reducing communication overhead through model compression and efficient communication protocols.

% This work also discusses the future research directions directions indicating that FRSs can provide more accurate personalized recommendations while better protecting user privacy. 
% Additionally, we showcase applications of FRS in various fields, demonstrating their potential and value in the real world. 
% Through this paper, we aim to provide a guidance for integrating FRS with FM, directing future research and technological advancements to collectively advance this field.

% The survey concludes that FRS enhanced by FM hold great promise for overcoming challenges such as data sparsity and privacy concerns. 
% By exploiting the generative capabilities of GMs such as DMs and LLMs, these systems can better mimic the underlying data distributions, potentially improving recommendation accuracy while preserving user privacy. 
% The integration of GMs into FRS represents a fertile ground for future research, promising advances in both theoretical understanding and practical applications. 
% This review aims to stimulate further exploration and development in this innovative and important area, encouraging researchers to address the challenges identified and explore the future directions outlined.

==> sections/sec_dir.tex <==
%!TEX root = ../main.tex


\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.85\columnwidth]{figures/dir.pdf}
    \caption{
        Key future directions for integrating FMs into FRSs aim to address emerging challenges and opportunities, focusing on enhancing recommendation performance, safeguarding user privacy, and improving system adaptability.
        }
    \label{fig:dir}
 \end{figure}   


\section{Future Directions}
\label{sec:dir}

As shown in Fig.~\ref{fig:dir}, The convergence of FMs and FRSs opens a promising yet challenging frontier. 
By harnessing the powerful representation capabilities of FMs alongside the privacy-preserving strengths of FRSs, researchers can transcend longstanding obstacles such as data sparsity and heterogeneity, while simultaneously boosting recommendation performance. 
In this section, we outline several critical future directions that not only exploit the intrinsic advantages of FMs but also address the new challenges they introduce. 
These directions serve as a comprehensive roadmap for advancing research and practical applications toward more robust and privacy-preserving recommendation services.

\subsection{Data Augmentation}
Data scarcity is a pervasive challenge in FRSs due to stringent privacy constraints that confine user data to local devices. 
Generative FMs, including Large Language Models and Diffusion Models, offer a compelling solution by synthesizing realistic user interaction data to augment training sets~\cite{feng2021survey,yang2022image}. 
By generating virtual interaction records and detailed item descriptions, these models can enrich sparse user profiles, thereby enhancing recommendation accuracy and personalization~\cite{yan2019differentiated}. 
Nonetheless, the quality of synthetic data must be rigorously validated to mitigate potential biases and noise~\cite{maharana2022review,li2019insufficient}. 
Moreover, integrating differential privacy techniques during data generation can ensure that sensitive user information remains protected. 
Future research should focus on developing robust methods for generating diverse and high-quality synthetic data, tailored to cover a wide range of user behaviors and scenarios.

\subsection{Cold-Start Recommendation}
The cold-start problem—stemming from insufficient historical interaction data for new users or items—remains a significant hurdle in FRSs~\cite{schein2002methods}. 
Pre-trained FMs, endowed with rich semantic knowledge from vast textual corpora, can generate high-quality representations for both users and items, thereby enabling zero-shot and few-shot learning approaches~\cite{gong2023unified,zhang2024federated}. 
This capability not only mitigates the cold-start issue but also facilitates a smoother adaptation to novel scenarios. However, ensuring robust privacy in federated settings and effectively transferring knowledge across domains without compromising model integrity remain challenging. 
Future work must advance privacy-preserving mechanisms and efficient knowledge transfer techniques to further bolster cold-start recommendations while maintaining stringent privacy standards~\cite{yu2024unleashing}.

\subsection{Multi-Modal Recommendation}
One of the standout strengths of FMs is their ability to process and integrate multiple data modalities, such as text, images, audio, and video, to construct richer and more nuanced user profiles~\cite{bommasani2021opportunities}. 
Incorporating multi-modal data into FRSs can lead to significantly enhanced personalization and recommendation quality~\cite{li2024personalized,geng2023personalized,huang2024foundation}. 
However, the inherent heterogeneity of different data types poses a considerable challenge in terms of unified representation. 
Future research should focus on developing sophisticated methods to map diverse modalities into a common latent space, while concurrently designing robust, privacy-preserving protocols to safeguard sensitive multi-modal information~\cite{wang2021survey,li2024personalized,feng2024robust,wu2024towards}.

\subsection{Real-Time Recommendations}
Real-time recommendation systems are crucial for dynamically adapting to evolving user behaviors and contextual cues~\cite{huang2015tencentrec}. 
FMs can enhance the accuracy and relevance of these recommendations by leveraging their advanced contextual understanding to process user queries and item descriptions in real time. 
Nevertheless, the high computational demands of FMs may introduce latency, adversely affecting the user experience. 
Future research should prioritize the development of model compression and acceleration techniques, such as knowledge distillation~\cite{kang2022personalized} and pruning~\cite{beel2019data}, to reduce computational complexity. 
Additionally, efficient context management strategies, e.g., sliding window approaches, should be explored to optimize the handling of continuous user behavior streams.

\subsection{Enhanced Explainability}
Explainability is pivotal for fostering user trust and satisfaction in recommendation systems. Language FMs, pre-trained on extensive textual datasets, are well-equipped to generate coherent, natural language explanations that elucidate the rationale behind recommendations~\cite{hada2021rexplug,geng2022path,liu2023chatgpt}. However, the computational cost of producing detailed explanations and the risk of perpetuating biases from pre-training data present significant challenges~\cite{bommasani2021opportunities,zhuang2023foundation}. Future research should aim to balance the trade-off between explanation quality and computational efficiency through model optimization and debiasing techniques. Moreover, incorporating user feedback into the explanation generation process can further refine and enhance the fairness and clarity of the recommendations.

\subsection{Advanced Metrics}
Evaluating FRSs integrated with FMs necessitates the development of advanced metrics that extend beyond conventional measures like rating prediction accuracy and item ranking~\cite{xu2024survey,wu2023survey}. Given the generative and explanatory capabilities of FMs, new evaluation frameworks must capture dimensions such as diversity, fairness, contextual relevance, and overall user satisfaction. Future work should focus on establishing comprehensive and holistic evaluation criteria that provide deeper insights into the performance of these hybrid systems, thereby guiding further optimization and innovation.

In summary, the integration of Foundation Models into Federated Recommendation Systems heralds a transformative shift toward more intelligent, adaptable, and privacy-conscious recommendation services. While the potential benefits are substantial, addressing the associated challenges—ranging from data quality and computational efficiency to privacy and fairness—requires a concerted research effort. The future directions outlined above offer a strategic roadmap for pioneering advancements in this emerging field, paving the way for next-generation recommendation systems that are both robust and user-centric.

==> sections/sec_intro.tex <==
%!TEX root = ../main.tex

\section{Introduction}
\label{sec:intro}

In today's digital era, the exponential growth of online information demands recommendation systems (RSs) that can efficiently filter, navigate, and personalize content for individual users. 
Traditional RSs have achieved significant success by tailoring products, content, and services to user preferences~\cite{ko2022survey}. 
However, their heavy reliance on centralized data collection not only raises serious privacy concerns, especially under stringent regulations like GDPR~\cite{voigt2017eu}, but also introduces operational bottlenecks.
%
To mitigate these issues, Federated Learning (FL) has emerged as a transformative paradigm that enables model training across distributed devices while keeping user data localized~\cite{mcmahan2017communication}. 
By leveraging the computational resources of individual devices, FL alternates between local model updates and global parameter aggregation, giving rise to Federated Recommendation Systems (FRSs) that preserve user privacy~\cite{zhang2021survey}. 
Despite these advantages, FRSs face two critical challenges: 
(a) severe data sparsity: since each client typically contains data from a single user with only a limited set of interactions;
and (b) significant data heterogeneity arising from diverse user behaviors and preferences. 
These challenges often lead to sub-optimal recommendation performance.
%
In parallel, the recent advent of Foundation Models (FMs) has revolutionized the field of artificial intelligence. 
Language Models such as ChatGPT~\cite{openai2022chatgpt}, vision models like ViT \cite{dosovitskiy2020image}, and multi-modal models like CLIP~\cite{radford2021learning} have demonstrated the power of pre-training on massive, diverse datasets. 
Through techniques such as \textbf{Fine-Tuning}~\cite{zhang2024scaling} and \textbf{Prompting}~\cite{gu2023systematic}, these models can be efficiently adapted to a wide range of downstream tasks, achieving state-of-the-art performance across various domains \cite{bommasani2021opportunities}. \looseness=-1

The integration of FMs into FRSs presents a promising avenue to address the challenges of data sparsity and heterogeneity \cite{zhang2024transfr}: 
First, the rich, pre-trained representations provided by FMs can compensate for the limited local data available on each client, thereby enhancing recommendation accuracy. 
Second, the generalization capabilities of FMs help alleviate the cold-start problem by leveraging learned patterns that are broadly applicable to new users and items. 
Third, the transfer learning strengths of FMs allow for rapid adaptation to new recommendation scenarios with minimal additional training. 
Moreover, by reducing the reliance on extensive data sharing, FM-based approaches inherently balance privacy protection with performance, while also mitigating communication overhead \cite{ren2024advances}. 

Despite these advantages, the fusion of FMs and FRSs is still in its early stages. Critical issues such as the privacy--performance trade-off, communication efficiency, and model fairness remain underexplored. In this paper, we introduce a lightweight FM adaptation framework tailored for federated environments. Our framework is designed to harness the pre-training benefits of FMs while navigating the constraints imposed by federated settings. We systematically analyze the challenges associated with this integration and propose future research directions aimed at overcoming these hurdles.

By bridging the gap between foundation models and federated recommendation systems, our work not only advances the state-of-the-art in privacy-preserving recommendation technologies but also lays the groundwork for innovative research at the intersection of these two paradigms.


==> sections/sec_related.tex <==
%!TEX root = ../main.tex





==> sections/sec_res.tex <==
%!TEX root = ../main.tex

\section{Resources}
\label{sec:res}

In this section, we introduce the commonly used datasets and evaluation metrics in FRS. 
The aim is to provide a comprehensive overview of the resources used in the field, helping readers understand the types of materials and benchmarks typically employed. 
This section presents various datasets, including explicit and implicit feedback types, along with metrics for evaluating recommendation performance. 
These datasets and metrics are crucial for assessing and improving the effectiveness of FRSs.

\subsection{Datasets}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/type_feedback.png}
    \caption{Two types of Feedbacks.}
    \label{fig:type_feedback}
\end{figure}


\begin{table*}[!htbp]
\centering
\caption{Datasets with Explicit Feedback.}
\resizebox{.95\textwidth}{!}{
\begin{tabular}{clcccccccc}
\hline
                            & \multicolumn{1}{c}{}                          &                          &                          &                              &                            & \multicolumn{4}{c}{Context}                                                                                                                   \\
\multirow{-2}{*}{}          & \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multirow{-2}{*}{\#User} & \multirow{-2}{*}{\#Item} & \multirow{-2}{*}{\#Feedback} & \multirow{-2}{*}{Sparsity} & User                              & Item                              & Feedback                          & Timestamp                         \\ \hline
                            & Amazon Beauty                                 & 1,210,271                & 249,274                  & 2,023,070                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Books                                  & 8,026,324                & 2,330,066                & 22,507,155                   & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon CDs                                    & 1,578,597                & 486,360                  & 3,749,004                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Cell Phone                             & 2,261,045                & 319,678                  & 3,447,249                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Clothing                               & 3,117,268                & 1,136,004                & 5,748,920                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Games                                  & 826,767                  & 50,210                   & 1,324,753                    & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Garden                                 & 714,791                  & 105,984                  & 993,490                      & 99.99\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   & {\color[HTML]{00B050} \checkmark} \\
                            & Amazon Home                                   & 2,511,610                & 410,243                  & 4,253,926                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Kindle                                 & 1,406,890                & 430,530                  & 3,205,467                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Movies                                 & 2,088,620                & 200,941                  & 4,607,047                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Music                                  & 478,235                  & 266,414                  & 836,006                      & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Sports                                 & 1,990,521                & 478,898                  & 3,268,695                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Amazon Toys                                   & 1,342,911                & 327,698                  & 2,252,771                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-14}{*}{Amazon Reviews}   & Amazon Video                                  & 426,922                  & 23,965                   & 583,933                      & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & ML-100K                                       & 943                      & 1,682                    & 100,000                      & 93.70\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & ML-1M                                         & 6,040                    & 3,952                    & 10,000,209                   & 95.81\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & ML-10M                                        & 69,878                   & 10,681                   & 10,000,054                   & 98.69\%                    & {\color[HTML]{00B050} \textbf{}}  & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-4}{*}{MovieLens} & ML-20M                                        & 138,493                  & 27,278                   & 20,000,263                   & 99.47\%                    & {\color[HTML]{00B050} \textbf{}}  & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & Yelp2018                                      & 1,326,101                & 174,567                  & 5,261,669                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2020                                      & 1,968,703                & 209,393                  & 8,021,122                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2021                                      & 2,189,457                & 160,585                  & 8,635,403                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yelp2022                                      & 1,987,929                & 150,346                  & 6,990,280                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-5}{*}{Yelp}      & Yelp-full                                     & 5,556,436                & 539,254                  & 28,908,240                   & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                            & Anime                                         & 73,515                   & 11,200                   & 7,813,737                    & 99.05\%                    &                                   & {\color[HTML]{00B050} \checkmark} &                                   &                                   \\
                            & Book Crossing                                 & 105,284                  & 340,557                  & 1,149,780                    & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                            & Douban                                        & 738,701                  & 28                       & 2,125,056                    & 89.73\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Epinions                                      & 116,260                  & 41,269                   & 188,478                      & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                            & Goodreads                                     & 876,145                  & 2,360,650                & 228,648,342                  & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Jester                                        & 73,421                   & 101                      & 4,136,360                    & 44.22\%                    &                                   &                                   &                                   &                                   \\
                            & Netflix                                       & 480,189                  & 17,770                   & 100,480,507                  & 98.82\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                            & Yahoo Music                                   & 1,948,882                & 98,211                   & 11,557,943                   & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\ \hline
\end{tabular}
}
\label{tab:explicit}
\end{table*}


\begin{table*}[!htbp]
\centering
\caption{Datasets with Implicit Feedback.}
\resizebox{.95\textwidth}{!}{
\begin{tabular}{clcccccccc}
\hline
                         & \multicolumn{1}{c}{}                          &                          &                          &                              &                            & \multicolumn{4}{c}{Context}                                                                                                                   \\
\multirow{-2}{*}{}       & \multicolumn{1}{c}{\multirow{-2}{*}{Dataset}} & \multirow{-2}{*}{\#User} & \multirow{-2}{*}{\#Item} & \multirow{-2}{*}{\#Feedback} & \multirow{-2}{*}{Sparsity} & User                              & Item                              & Feedback                          & Timestamp                         \\ \hline
                         & MIND\_large\_train                            & 711,223                  & 27,047                   & 83,507,374                   & 99.57\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & MIND\_large\_dev                              & 255,991                  & 6,998                    & 14,085,557                   & 99.21\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & MIND\_small\_train                            & 50,001                   & 20,289                   & 5,843,444                    & 99.42\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
\multirow{-4}{*}{MIND}   & MIND\_small\_dev                              & 50,001                   & 5,370                    & 2,740,998                    & 98.98\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\ \hline
                         & QK-video                                      & 5,022,750                & 3,753,436                & 142,321,193                  & 99.99\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                         & QK-article                                    & 1,325,838                & 220,122                  & 46,111,728                   & 99.98\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
                         & QB-video                                      & 34,240                   & 130,647                  & 1,701,171                    & 99.96\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\
\multirow{-4}{*}{Tenrec} & QB-article                                    & 24,516                   & 7,355                    & 348,736                      & 99.81\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} &                                   &                                   \\ \hline
                         & Adressa                                       & 15,514                   & 923                      & 2,717,915                    & 81.02\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Foursquare                                    & 1,083                    & 38,333                   & 227,428                      & 99.45\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Gowalla                                       & 196,591                  & 950,327                  & 6,442,890                    & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} \checkmark} & {\color[HTML]{00B050} \checkmark} \\
                         & Last.FM                                       & 1,892                    & 17,632                   & 92,834                       & 99.72\%                    &                                   &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} \\
                         & Pinterest                                     & 55,187                   & 9,911                    & 1,445,622                    & 99.74\%                    &                                   &                                   &                                   &                                   \\
                         & Steam                                         & 2,567,538                & 32,135                   & 7,793,069                    & 99.99\%                    &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                         & TaFeng                                        & 32,266                   & 23,812                   & 817,741                      & 99.89\%                    & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\
                         & Tmall                                         & 963,923                  & 2,353,207                & 44,528,127                   & 99.99\%                    &                                   &                                   & {\color[HTML]{00B050} $\checkmark$} & {\color[HTML]{00B050} $\checkmark$} \\ \hline
\end{tabular}
}
\label{tab:implicit}
\end{table*}

As shown in Fig. \ref{fig:type_feedback}, the datasets used can be categorized into two types based on user feedback in FRS: explicit feedback and implicit feedback.
Explicit feedback includes direct responses from users about their preferences. 
This typically includes ratings (such as a 1-5 scale), user comments, and like/dislike statements. 
Such data provides straightforward insights into user preferences, making it highly valuable for training recommendation models.
Common datasets with explicit feedback include the following shown in Table~\ref{tab:explicit}: 
\begin{itemize}
    \item Amazon Reviews\footnote{https://cseweb.ucsd.edu/~jmcauley/datasets.html\#amazon\_reviews}: The Amazon Reviews dataset is a large-scale dataset that contains product information across various categories such as Books, CDs, and Music. It includes reviews (ratings, text, helpfulness votes) and product metadata (description, category information, price, brand, and image features). There are three updated versions of this dataset from the years 2014~\cite{mcauley2015image,he2016ups}, 2018~\cite{ni2019justifying}, and 2023~\cite{hou2024bridging}.
    \item MovieLens Datasets\footnote{https://grouplens.org/datasets/movielens/}: The MovieLens datasets~\cite{harper2015movielens}, initially released in 1998, capture individuals' stated movie preferences. These preferences are recorded as tuples, with each tuple showing a person's rating (from 0 to 5 stars) for a movie at a specific time. Users enter these ratings through the MovieLens website, which provides personalized movie suggestions based on these ratings.
    \item Yelp Datasets\footnote{https://www.yelp.com/dataset}: This dataset is a subset of Yelp's business, review, and user data. It was initially developed for the Yelp Dataset Challenge, which allows students to study or analyze Yelp data and present their insights. In total, there are four versions of the Yelp datasets.
    \item Anime\footnote{https://www.kaggle.com/datasets/CooperUnion/anime-recommendations-database}: It collects user preference data from the MyAnimeList website, and contains information from 73,516 users on 12,294 anime titles. Users can add anime to their completed list and rate them, and this dataset compiles these ratings.
    \item Book Crossing\footnote{https://grouplens.org/datasets/book-crossing/}: The Book-Crossing dataset is a well-structured collection of data collected by Cai-Nicolas Ziegler in a 4-week crawl from the Book-Crossing community. This dataset primarily comprises user interactions that include book ratings, ranging from 0 to 10. 
    \item Douban\footnote{https://www.kaggle.com/datasets/utmhikari/doubanmovieshortcomments}: The Douban Movie dataset is a Chinese website where internet users can post their opinions and comments about films. It contains over 2 million short comments on 28 movies from the Douban Movie website.
    \item Epinions\footnote{https://cseweb.ucsd.edu/~jmcauley/datasets.html\#social\_data} \cite{cai2017spmc}: This dataset was collected from Epinions.com, a popular online consumer review site. It includes trust relationships between users and covers a period from January 2001 to November 2013.
    \item Goodreads\footnote{https://www.kaggle.com/datasets/jealousleopard/goodreadsbooks}: This dataset includes reviews from the book review website Goodreads, along with various attributes describing the books. Importantly, the dataset captures different levels of user interaction, from adding books to a shelf, to rating them, to reading them.
    \item Jester\footnote{https://eigentaste.berkeley.edu/dataset/}: It focuses exclusively on jokes. Users of the Jester online platform rate jokes and these ratings are then used to personalize joke recommendations for them.
    \item Netflix\footnote{https://www.kaggle.com/datasets/netflix-inc/netflix-prize-data}: Netflix provided a training dataset consisting of 100,480,507 ratings from 480,189 users for 17,770 films. The user and the movie are identified by integer IDs, and the rating scores range from 1 to 5 stars, also as integers.
    \item Yahoo Music\footnote{https://webscope.sandbox.yahoo.com/catalog.php?datatype=r}: It is known for its diversity and large scale. It contains a large collection of user ratings on different musical elements such as artists and genres.
\end{itemize}

Implicit feedback, on the other hand, is derived from user actions that indirectly indicate preferences, such as bookmarks, video/music play history, or click-throughs. Although implicit feedback does not directly express user likes or dislikes, it is rich and captures user behaviour more comprehensively.
\begin{itemize}
    \item MIND\footnote{https://msnews.github.io/}~\cite{wu2020mind}: The MIND dataset, sourced from the Microsoft News website, is a large-scale collection of approximately 160,000 English news articles and over 15 million user interaction records. It has been designed to advance research in news recommendation systems. It includes detailed textual content for each story and anonymized user interaction data to ensure privacy.
    \item Tenrec\footnote{https://github.com/yuangh-x/2022-NIPS-Tenrec}~\cite{yuan2022tenrec}: The Tenrec dataset is a comprehensive benchmark dataset for RSs, featuring user interactions from two recommendation platforms across four dataset files: QK-video and QB-video for video actions, and QK-article and QB-article for article actions.
    \item Adressa\footnote{https://reclab.idi.ntnu.no/dataset/}~\cite{gulla2017adressa}: It is a corpus of Norwegian news articles related to anonymous users. It is a collaborative project between the Norwegian University of Science and Technology and Adressavisen. The objective is to gain insight into the nature of news articles and their readers.
    \item Foursquare\footnote{https://sites.google.com/site/yangdingqi/home/foursquare-dataset}~\cite{yang2014modeling}: This dataset comprises check-in data from New York City, collected over a period of approximately ten months (from 12 April 2012 to 16 February 2013). It encompasses 227,428 check-ins in New York City, with each check-in recorded with its timestamp, GPS coordinates, and detailed venue category.
    \item Gowalla\footnote{https://snap.stanford.edu/data/loc-gowalla.html}~\cite{cho2011friendship}: Gowalla is a location-based social networking website where users can post their whereabouts by checking in. The dataset comprises data collected from the public API, which represents an undirected friendship network with 196,591 nodes and 950,327 connections. Additionally, it records 6,442,890 check-ins made by these users between February 2009 and October 2010.
    \item Last.FM\footnote{https://grouplens.org/datasets/hetrec-2011/}~\cite{Cantador:RecSys2011}: The Last.FM dataset represents a valuable resource that has been extensively utilized in the field of music information retrieval and RSs. It captures detailed information regarding music listening events from users. Each listening event is further enhanced with user demographics and specific descriptors that reflect their music tastes and consumption behaviours. 
    \item Pinterest\footnote{https://github.com/edervishaj/pinterest-recsys-dataset}~\cite{geng2015learning}: The Pinterest dataset represents a valuable resource for a variety of research and analytical purposes. It encompasses a diverse range of data, including images, user features, interests, and user interactions. 
    \item Steam\footnote{https://github.com/kang205/SASRec}~\cite{kang2018self}: Steam is a collection of information about games published on the Steam platform. It includes details such as game names, release dates, genres, developers, publishers, and other relevant information. 
    \item TaFeng\footnote{https://www.kaggle.com/datasets/chiranjivdas09/ta-feng-grocery-dataset}: TaFeng is a comprehensive collection of supermarket shopping data, including detailed transaction records from the Ta Feng supermarket in Taiwan, covering a period from November 2000 to February 2001. The dataset comprises a variety of data points, including customer demographics, product categories, and detailed item descriptions along with quantities purchased.
    \item Tmall\footnote{https://tianchi.aliyun.com/dataset/53}\cite{tmall18dataset}: The Tmall dataset is a comprehensive collection from Tmall, comprising anonymized user shopping records over a six-month period up to and including the "Double 11" event. It should be noted that the data is selectively sampled to address privacy concerns.
\end{itemize}

Both types of feedback play a critical role in the development of FRSs, providing diverse insights into user preferences that help improve the recommendation accuracy and relevance.


\begin{figure*}[!t]
    \centering
    \includegraphics[width=.95\textwidth]{figures/framework.pdf}
    \caption{
        A potential unified framework for FRSs integrates server-side global aggregation and hyperparameter optimization with client-side data processing, model training, and evaluation.
        }
    \label{fig:framework}
 \end{figure*}   


\subsection{Metrics}
\label{sec:metrics}

In the field of FRSs, the use of evaluation metrics is fundamental to assessing and refining the performance of our algorithms. Metrics serve as a quantitative lens through which we can observe how closely the system's suggestions match users' actual interests and preferences.

For predicting how well a system can estimate user preferences, there are several metrices measuring the prediction errors to judge the accuracy of the predictions \cite{shani2011evaluating}, such as Mean Absolute Error, Mean Squared Error and Root Mean Squared Error.
When it comes to classifying items, i.e., determining whether a user will like a product or not, we look at metrics such as Precision, Recall, Hit Ratio, F1 Score, Accuracy and AUC. 
These tell us how correctly the RS is classifying items, and the F1 score helps us balance the Precision and Recall.
%
Then to measure the item ranking ability, which is about listing recommendations in the right order, Average Precision and Mean Average Precision are key to this, as they assess the quality of the order of recommendations. 
Metrics such as Mean Reciprocal Rank \cite{voorhees2001trec}, Normalized Mutual Rank \cite{flanagan2021federated} and Normalised Discounted Cumulative Gain \cite{he2015trirank} also contribute by assessing how well the top recommended items are ranked.

On a broader scale, we consider recommendation-centric metrics such as Diversity, which ensures that a variety of items are suggested, and Coverage, which measures how many items from the catalogue are recommended. There are also some user-centric metrics include Novelty, which measures how new or surprising the recommendations are, and Degree of Agreement (DOA) \cite{wu2021hierarchical}, which quantifies the level of concordance between the ranking of items produced by a recommendation system and the ranking preferred by the user. 
Moreover, business metrics such as Click-Through Rate \cite{bian2023feynman} are critical to assessing the system's impact on user engagement and the company's bottom line, and Conversion Rate \cite{bian2023feynman} measures how efficient an algorithm is at providing recommendations that lead to user purchases.
There also are some metrics for measuring other functionality. 
For example, Gini Index \cite{castells2021novelty} evaluates the fairness of recommendation distribution, with lower values indicating more equitable distribution across items.



\subsection{Open-source framework}


Although there are already mature open-source frameworks for both RSs \cite{zhou2023mmrec,recbole[1.0],recbole[2.0],recbole[1.2.0]} and FL \cite{beutel2020flower,liu2021fate,openfl_citation}, there remains a significant gap when it comes to FRSs. 
Currently, there is no mature, unified, and widely applicable open-source framework specifically designed for FRSs.
%
Efforts such as FedMR\footnote{https://github.com/mtics/FedMR} \cite{li2024personalized} attempt to bridge this gap by integrating features from existing frameworks like MMRec\footnote{https://github.com/enoche/MMRec} \cite{zhou2023mmrec} and RecBole\footnote{https://github.com/RUCAIBox/RecBole} \cite{zhou2023mmrec}, extending them into the realm of federated multimodal recommendation. 
However, FedMR is still in its infancy and does not yet provide the robustness or general applicability required of a comprehensive solution for FRSs.

As illustrated in Fig. \ref{fig:framework}, we make a preliminary attempt to propose a potential unified framework for FRSs in this paper, which aims to ideally encompass the following:

\begin{itemize}
    \item \textbf{Integration of RSs and FL}: 
    Such a framework should seamlessly integrate the strengths of traditional recommendation systems with privacy-preserving capabilities from federated learning, addressing both data heterogeneity and privacy constraints effectively.
    
    \item \textbf{Modular and Extensible Architecture}: 
    The framework should feature a modular design that separates core components such as data preprocessing, model training, evaluation, and aggregation, facilitating improvements and the easy integration of new modules or functionalities.
    
    \item \textbf{Support for Multimodal Data}: 
    Leveraging the strengths of multimodal models, the framework should support the incorporation of various data modalities, enabling a more comprehensive understanding of user preferences and improving recommendation accuracy.
    
    \item \textbf{Scalability and Device Adaptability}: 
    The framework must be capable of scaling to accommodate a large number of clients and adapt to heterogeneous devices with varying computational capabilities, ensuring efficient performance on resource-constrained devices.
    
    \item \textbf{Privacy and Security}: 
    The framework should incorporate advanced privacy-preserving mechanisms, such as differential privacy and secure multi-party computation, to guarantee data confidentiality during both training and communication phases.
\end{itemize}

Despite the absence of a mature open-source FRS framework, the existing building blocks in RS and FL frameworks provide a strong foundation. 
By extending these capabilities and overcoming the unique challenges posed by FRSs, our proposed framework serves as a step towards a widely adopted, unified solution that fully supports FRSs.


% \begin{itemize}
%     \item Integration of Recommendation and Federated Learning: Such a framework should seamlessly integrate the strengths of traditional recommendation systems with privacy-preserving capabilities from federated learning, addressing both data heterogeneity and privacy constraints effectively.

%     \item \textbf{Modular and Extensible Architecture:} The framework should feature a modular design that separates core components such as data preprocessing, model training, evaluation, and aggregation. This separation would facilitate improvements and the easy integration of new modules or functionalities.

%     \item \textbf{Support for Multimodal Data:} Leveraging the strengths of multimodal models, the framework should support the incorporation of various data modalities (e.g., text, images, audio), enabling a more comprehensive understanding of user preferences and improving recommendation accuracy.

%     \item \textbf{Scalability and Device Adaptability:} The framework must be capable of scaling to accommodate a large number of clients and adapt to heterogeneous devices with varying computational capabilities. Techniques like model compression and lightweight fine-tuning should be employed to ensure efficient performance on resource-constrained devices.

%     \item \textbf{Privacy and Security:} The framework should incorporate advanced privacy-preserving mechanisms, such as differential privacy and secure multi-party computation, to guarantee data confidentiality during both training and communication phases.

% \end{itemize}

% Despite the absence of a mature open-source FRS framework, the existing building blocks in RS and FL frameworks provide a strong foundation. By extending these capabilities and overcoming the unique challenges posed by FRS, future work could lead to the development of a widely adopted, unified framework that fully supports federated recommendation scenarios.

==> sections/sec_tax.tex <==
%!TEX root = ../main.tex

\section{Federated Recommendation Systems with Foundation Models}
\label{sec:frs_w_fm}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=1.\columnwidth]{figures/frs_fm.pdf}
    \caption{
        Integration framework of FRSs with FMs, illustrating the key challenges across three stages: Client Model Update, Communication, and Global Aggregation.
    }
    \label{fig:frs_fm}
\end{figure}

Figure~\ref{fig:frs_fm} presents the integration framework of FRSs with FMs, delineating three pivotal stages: client model update, communication, and global aggregation~\cite{alamgir2022federated}. 
In this section, we provide an in-depth discussion of each stage, emphasizing how FMs can address core challenges in FRSs such as data sparsity, heterogeneity, and privacy preservation.

\subsection{Client Model Update}
The client model update stage in FRSs is inherently challenged by the unique characteristics of decentralized data and device constraints~\cite{yang2020federated,alamgir2022federated}, which posits three key issues:

\noindent \textbf{Data Sparsity}:  
Due to stringent privacy requirements, user data, including interaction histories and personal profiles, remains on local devices, forming isolated data silos. 
Although this approach complies with privacy regulations and bolsters user trust, it also means that each client possesses only a limited subset of the overall dataset. 
Consequently, data sparsity becomes a significant barrier to model performance. 

\noindent \textbf{Non-IID Data}:  
Since each client independently trains the model on its localized data, the aggregated data distribution is inherently non-independent and identically distributed (non-IID). 
This heterogeneity reflects the diverse preferences and behaviors of users, which, while enhancing personalization, complicates the training process and model convergence.

\noindent \textbf{Device Limitations}:  
Clients typically operate on consumer-grade devices such as smartphones that have limited computational resources, and may experience unstable connectivity. 
Therefore, the local model’s computational burden and the volume of information exchanged must be minimized.

FMs, pre-trained on vast and diverse datasets, offer robust representational capabilities that can be efficiently fine-tuned to local conditions~\cite{bommasani2021opportunities}. 
Thus, integrating FMs in the client update phase yields several advantages:

\noindent \textbf{Addressing Data Sparsity}:
By leveraging transfer learning, FMs can apply knowledge gained from large corpora to the sparse local datasets~\cite{zeng2024federated}. 
Fine-tuning a FM on limited client data enables effective adaptation to individual user behaviors, leading to improved recommendation accuracy~\cite{wu2023survey,yuan2024fellas}. 
Crucially, local fine-tuning ensures that sensitive data remains on the device, thereby preserving privacy~\cite{rame2023model}. \looseness=-1

\noindent \textbf{Handling Non-IID Data}: FMs possess powerful semantic understanding that allows them to capture complex patterns and nuances from non-IID data. Their ability to interpret diverse inputs, such as search queries~\cite{lu2020twinbert,liu2021pre}, user comments~\cite{liu2023pre}, and other textual signals~\cite{geng2022recommendation}, enables a more personalized recommendation process, effectively mitigating the challenges of data heterogeneity~\cite{han2021pre,li2024feddae,tang2024higpt}.

\noindent \textbf{Adapting to Device Limitations}: Although fine-tuning FMs can be computationally demanding, recent advances in lightweight fine-tuning techniques and model compression have substantially reduced the computational overhead~\cite{han2024parameter,chen2024percept,zhu2023survey}. This allows FMs to deliver enhanced performance even on resource-constrained devices.

Overall, by integrating FMs during the client update stage, FRSs can overcome inherent limitations related to data sparsity, non-IID distributions, and device constraints, thereby significantly enhancing local model performance.

\subsection{Communication}

The communication phase, involving the transfer of model updates from clients to the central server, is critical for maintaining both system performance and user privacy. However, it would face two main challenges:

\noindent \textbf{High Communication Costs}:  
Transmitting high-dimensional model parameters, gradients, or other statistical summaries from numerous clients can impose substantial communication overhead, especially in large-scale systems where bandwidth and latency are constrained.

\noindent \textbf{Transmission Security}:  
Model updates often contain sensitive information that could compromise user privacy. 
While encryption and secure aggregation techniques exist, they generally add to the computational and communication burdens.

FMs offer promising solutions to these challenges by leveraging their advanced representation and compression capabilities. 
FMs are typically pre-trained on large, diverse datasets, providing them with rich knowledge and strong representational capabilities. 
This pre-training endows them with prior knowledge that can be quickly adapted to specific client data through fine-tuning \cite{bommasani2021opportunities}. 
Therefore, FMs learn general feature representations, offering adaptability to different data distributions. 
Applying FMs during the client update phase in FRS can significantly enhance the performance of local models. 
Specifically, the advantages are outlined as follows:

\noindent \textbf{Addressing Data Sparsity}: 
FMs can apply the knowledge learned from large corpora to local data through transfer learning \cite{zeng2024federated}. 
For instance, a pre-trained FM can be effectively fine-tuned on a small amount of local data at the client to adapt to specific user behaviors, thereby achieving good performance in downstream tasks such as providing more accurate recommendations \cite{wu2023survey,yuan2024fellas}. 
Furthermore, by fine-tuning the base model locally, sensitive data does not need to leave the device, protecting user privacy \cite{rame2023model}. 
Thus, even with limited data, clients can achieve better model performance, alleviating the challenges brought by data sparsity.

\noindent \textbf{Handling Non-IID Data}: FMs' strong representational capabilities enable them to capture complex user preferences and behaviors. 
For example, FMs possess powerful semantic understanding abilities, allowing them to better interpret user search queries \cite{lu2020twinbert,liu2021pre}, comments \cite{liu2023pre}, and other textual data \cite{geng2022recommendation}, thereby providing recommendations that align more closely with user needs. 
Moreover, FMs can learn complex patterns from non-IID data \cite{han2021pre,li2024feddae,tang2024higpt}, enhancing the model's adaptability to different user preferences and ensuring that recommendation results stay consistent with the user's current interests and needs. 
Applying FMs during the client update phase can achieve a higher level of personalized recommendation, effectively addressing data heterogeneity.

\noindent \textbf{Adapting to Device Limitations}: 
Although fine-tuning and updating FMs typically require significant computational resources, optimizing the model architecture and employing lightweight fine-tuning techniques can reduce the computational burden on devices \cite{han2024parameter}. 
The knowledge transfer capability of FMs allows for efficient local fine-tuning under limited computational resources, thereby achieving good recommendation performance even in resource-constrained environments \cite{chen2024percept,han2024parameter}. 
Additionally, model compressions can be used to reduce the model size, thereby improve communication efficiency to suit the limitations of user devices \cite{zhu2023survey}.


\subsection{Global Aggregation}

The global aggregation phase is responsible for synthesizing the diverse and heterogeneous updates received from clients into a cohesive global model. This stage is pivotal for ensuring the overall effectiveness of personalized recommendations, yet it must contend with several challenges:

\noindent \textbf{Diverse Client Updates}:  
Central servers must integrate updates from a wide array of clients, each with distinct data distributions and user behaviors. 
Effective aggregation is essential to maintain model quality and recommendation accuracy.

\noindent \textbf{Noisy Data}:  
Client updates may include noisy or anomalous data that can degrade the performance of the global model. Robust aggregation methods are required to filter out such inconsistencies without sacrificing valuable information.

\noindent \textbf{Scalability}:  
As the number of clients and the volume of data increase, the aggregation process must be highly scalable to ensure timely and efficient model updates.

Traditional methods such as the weighted averaging approach used in FedAvg~\cite{mcmahan2017communication} do not fully exploit the contextual richness of client updates. In contrast, FMs can enhance global aggregation through several innovative strategies:

\noindent \textbf{Context-Aware Aggregation}: 
FMs leverage their powerful representation capabilities to analyze structural and statistical characteristics of client updates, including update frequency, magnitude, and temporal trends, enabling the assignment of contextually appropriate weights to each update~\cite{yu2023federated}. This approach improves the fidelity of the global model by aligning the aggregation process with system-wide patterns.

\noindent \textbf{Dynamic Weighting}: 
FMs facilitate dynamic adjustments of update weights based on their relevance and contribution to global parameters, e.g., client updates with under-represented data distributions can be assigned higher weights to ensure the model remains comprehensive and robust~\cite{han2024parameter,duan2020self}.

\noindent \textbf{Knowledge-Based Aggregation}: 
By harnessing their extensive pre-trained knowledge, FMs can infer latent relationships and patterns from client updates, effectively compensating for sparse or inconsistent data. 
This knowledge-based approach enhances the aggregation process, particularly when certain clients provide insufficient data~\cite{rawte2023survey,chen2024large}.

\noindent \textbf{Anomaly Detection and Handling}: 
FMs excel at detecting anomalies in client updates by identifying deviations from typical patterns. 
By down-weighting or excluding anomalous updates, FMs help maintain the stability and robustness of the global model~\cite{elhafsi2023semantic,xu2024customizing,liu2023pre}.

Overall, the integration of FMs into the global aggregation phase empowers FRSs to intelligently synthesize diverse client updates. 
By incorporating context-aware analysis, dynamic weighting, knowledge-based inference, and robust anomaly handling, FMs significantly enhance the quality, robustness, and adaptability of the aggregated model. 
This positions FMs as a transformative tool for advancing personalized, scalable, and privacy-preserving recommendation systems. 
Continued research in this area promises further improvements, driving the evolution of FRSs toward more intelligent and secure systems.

